Finding Connected Components on Map-reduce in Logarithmic Rounds

Given a large graph G = (V,E) with millions of nodes and edges, how do we compute its connected components efficiently? Recent work addresses this problem in map-reduce, where a fundamental trade-off exists between the number of map-reduce rounds and the communication of each round. Denoting d the diameter of the graph, and n the number of nodes in the largest component, all prior map-reduce techniques either require d rounds, or require about n|V| + |E| communication per round. We propose two randomized map-reduce algorithms -- (i) Hash-Greater-To-Min, which provably requires at most 3log(n) rounds with high probability, and at most 2(|V| + |E|) communication per round, and (ii) Hash-to-Min, which has a worse theoretical complexity, but in practice completes in at most 2log(d) rounds and 3(|V| + |E|) communication per rounds. Our techniques for connected components can be applied to clustering as well. We propose a novel algorithm for agglomerative single linkage clustering in map-reduce. This is the first algorithm that can provably compute a clustering in at most O(log(n)) rounds, where n is the size of the largest cluster. We show the effectiveness of all our algorithms through detailed experiments on large synthetic as well as real-world datasets.

==> cc/algosDiff.tex <==
\section{Connected Components on Map-Reduce}
\label{sec:algos}
In this section, we present map-reduce algorithms for transitive closure. We start by describing the Tarjan's algorithm \cite{tarjan72:depth} for computing the connected components in a central setting of a graph (the transitive closure can in turn be computed from this output). The algorithm  starts a depth first search from an arbitrary node in the graph and assign every explored node to the current component.  The search does not explore a node twice; hence, it terminates when all the nodes in the current component are visited. The algorithm continues to find a new component by starting a depth first search from an arbitrary remaining node. The total complexity of the algorithm is $O(\nnodes+\nedges)$.

\subsection{General Map-reduce Algorithm}
\newcommand{\TC}{\ensuremath{\tilde{\C}}}
\begin{algorithm}[t]
\caption{General Map Reduce Algorithm}
\begin{algorithmic}[1]
\STATE {\bf Input:} A graph $G = (V,E)$, \newline
{\em hashing} function $\h$, \newline
{\em local aggregation} function $\Md$, and \newline
{\em export} function \export
\STATE {\bf Output:} A set of connected components $\C \subset 2^V$
\STATE Let $\TC$ map each vertex $v$ to its neighborhood $N(v)$ (i.e., $\TC(v) = N(v)$).
 \REPEAT
  \STATE {\bf Map:}
  \STATE  $\forall v \in V$ compute $\h(\TC(v))$
  \STATE  $\forall (C_u, u) \in \h(\TC(v))$, send message $C_u$ to machine $u$.
  \STATE {\bf Reduce for node $v$:}
  \STATE Let ${\cal S}_v$ denote the set of messages received by $v$.
  \STATE Set $\TC(v) \leftarrow \Md({\cal S}_v)$
 \UNTIL {$\TC$ does not change}
 \STATE Return $\C = \mbox{\export}(\TC)$
\end{algorithmic}
\label{algo:distributed}
\end{algorithm}

Algorithm~\ref{algo:distributed} outlines a general map-reduce algorithm framework for computing the connected components in a graph. The algorithm  is parameterized by two functions -- a {\em hashing} function $\h$ that specifies which messages are sent to the different reducers, and a {\em local aggregation} function $\Md$ that specifies how messages received at a reducer are aggregated. We will show later in the section different choices for $(\h, \Md)$ create algorithms that have very different communication and rounds complexity.

The algorithm framework starts with each node $v$ associated with a cluster of nodes $\TC(v)$ containing itself and all its neighbors $N(v)$ in $G$. These clusters are distributed to different machines; let $m(v)$ denote the machine that contains $\TC(v)$. In the map stage, each cluster $\TC(v)$ uses $\h$ to compute a set of {\em hashes} (or messages)  $(C_u, u)$, one for every node $u$ appearing in $\TC(u)$. These hashes are then sent to the respective clusters; i.e., $C_u$ is sent to $m(u)$. In the reduce stage, each node $u$ aggregates all the received messages $(C_u, u)$ to compute a new cluster $\TC(u)$. This process is repeated until there is no change to the clusters $\TC$.  Finally, an appropriate \export function computes the connected components $\C$ from the final clusters $\TC$ using one map-reduce step.

We describe four different hashing strategies below. We assume a total ordering on the nodes, and we say for two nodes $u,v$, that $u < v$ if implied by the ordering.  For a node $v$, $\TC(v)$ denotes the cluster at machine $m(v)$, and $v_{min}$  the {\em smallest} node~(as per the total ordering) in the cluster $\TC(v)$. Finally, let $\core(v) = \{u |  u \in \TC(v)~and~u > v\}$ be the set of nodes in $\TC(v)$ that are greater than $v$. Each hashing strategy describes what messages are sent from the machine $m(v)$.

\squishlist
\item \Hma: $\h$ sends the entire cluster $\TC(v)$ to $m(v)$ and $v_{\min}$ to $m(u)$ for all  $u \in \TC(v)$. %That is, $\h$ generates a set of messages $\{(\{v_{\min}\}, u) \mid u \in \TC(v)\}$, where $v_{\min}$ is the smallest node in $\TC(v)$.

\item \Ha:  $\h$ sends the entire cluster $\TC(v)$ to $m(u)$ for all $u \in \TC(v)$. %That is, the set of messages generated is $\{(\TC(v), u) \mid u \in TC(v) \}$.

\item \Hm: $\h$ sends the entire cluster $\TC(v)$  to $m(v_{\min})$, and $v_{\min}$ to $m(u)$ for all $u \in \TC(v)$.%; i.e., the set of messages is $\{(\TC(v), v_{\min})\} \cup \{(\{v_{\min}\}, u) \mid u \neq v_{\min} \in \TC(v)\}$.

\item \Hcm: $\h$ sends the entire set $\core(v)$ to $m(v_{\min})$, and  $v_{\min}$ to $m(u)$ for all $u \in \core(v)$. %; i.e., the set of messages is $\{(\core(v), v_{\min})\} \cup \{(\{v_{\min}\}, u) \mid u \neq v_{\min} \in \core(v)\}$.
\squishend

We also describe two merging functions $\Md$. Denote $message(u,v)$ the set of nodes sent from $m(u)$ to $m(v)$ using the hashing function. The goal of $\Md$ is to collect all incoming messages to the reducer $m(v)$ and compute the new $\TC(v)$.

\squishlist

\item \Ua: $\Md$ computes $\TC(v)$ as the union of all incoming sets $\cup_{u} message(u,v)$.

\item \Um: $\Md$ first computes the min of all incoming messages and adds it to the set $message(v,v)$ to computes $\TC(v)$.

\squishend

We next describe  four different implementations of Algorithm~\ref{algo:distributed} -- \Hma, \Ha, \Hm and \Hcm. We show that \Hma is identical to the implementation in Pegasus \cite{pegasus} and computes the connected components in $O(d)$ map-reduce steps and with $O(\nnodes + \nedges)$ communication. \Ha, \Hm, and \Hcm are our novel contributions. \red{(Is \Ha novel or is it the same as existing work? We say it is existing work in intro?)} \Ha and \Hcm provably compute the answer in just $O(\log d)$, $O(\log n)$ and $2\log d$ (conjectured) map-reduce iterations, respectively. We can show that \Ha uses $O(n \nnodes + \nedges)$ communication while \Hcm uses only $O(\nnodes + \nedges)$ communication (same as Pegasus). We conjecture that \Hm takes only $2 \log d$ map-reduce iterations, and this bound is demonstrated in our experiments.

\subsection{\Hma Algorithm}

\Hma associated a label with each node, and in every iteration a node adopts the minimum label in its neighborhood as its label. On convergence, nodes that share the same label are in the same connected component. This algorithm can be implemented in our framework as follows: foreach cluster $\TC(v)$, the hash function $\h$ computes the {\em smallest} node in its cluster and sends it to all the neighbors of $v$. That is, $\h$ generates a set of messages $\{(\{v_{\min}\}, u) \mid u \in \{v\} \cup N(v)\}$, where $v_{\min}$ is the smallest node in $\TC(v)$. The smallest node could, for instance, be the node with the smallest id.

 On receiving the messages, the local aggregation function $\Md$ computes the smallest node amongst the incoming messages and includes it in its cluster.  More formally, say $u_{\min}$ is the smallest nodes appearing in all the messages received by $u$, then $\TC(v)$ is updated to $\{u_{\min}\} \cup \{v\} \cup N(v)$.

 Finally, the connected components are computed by the following \export function. For each node $v$, we compute the smallest node appearing in its cluster $v_{\min}$. The connected components are just the sets of nodes that share the same $v_{\min}$.

 \begin{theorem}[\Hma~\cite{pegasus}]
Algorithm \Hma correctly computes the connected components of  $G = (V,E)$ using $O(\nnodes + \nedges)$ communication and $O(d)$ map-reduce rounds.
 \end{theorem}
 \eat{
 \begin{proof}(sketch)
 First, \Hma correctly computes the connected components since any node that is connected to the smallest node $u_{\min}$ via a shortest path of length $p$ gets $u_{\min}$ in exactly $p$ steps. This also shows that the algorithm requires $O(d)$ map-reduce steps, since in each step the smallest node travels one edge. Finally, the communication cost is $O(\nnodes+\nedges)$ since a breadth first search is simulated.
 \end{proof}
}

 \subsection{\Ha Algorithm}
 In \Ha, the hash function $\h$ sends the entire cluster $\TC(v)$ to every node in the cluster. That is, the set of messages generated is $\{(\TC(v), u) \mid u \in TC(v) \}$. On receiving the messages, $\Md$ updates the cluster by taking the union of all the clusters received by the node. More formally, if the node $u$ receives clusters $C_1, \ldots, C_k$, then $\TC(u)$ is updated to $\cup_{i = 1}^k C_i$.

 We can show that after $O(\log d)$ map-reduce iterations, for every $u$, $\TC(u)$ contains all the nodes in the connected component containing $u$. Hence, the \export function just returns the distinct sets in $\TC$ (using one map-reduce step).
 \begin{theorem}[\Ha]
Algorithm \Ha correctly computes the connected components of  $G = (V,E)$ using $O(n\nnodes + \nedges)$ communication and $\log d$ map-reduce rounds, where $n$ is the size of the largest component.
 \end{theorem}
 \begin{proof}(sketch)
 We can show using induction that after $k$ map-reduce steps, every node $u$ that is at a distance $\leq 2^k$ from $v$ is contained in $\TC(v)$. Initially this is true, since all neighbors are part of $\TC(v)$. Again, for the $k+1^{st}$ step,  $u \in \TC(u')$ for some $u'$ and $u' \in \TC(v)$ such that distance between $u, u'$ and $u', v$ is at most $2^k$. Hence, for every node $u$ at a distance at most $2^{k+1}$ from $v$, $u \in TC(v)$ after $k+1$ steps.
 \end{proof}
\red{(1) Need proof of communication complexity. (2) Need a sentence which says this is similar to existing work ?? }

 \subsection{\Hm Algorithm}
 While the \Ha algorithm computes the connected components in a smaller number of map-reduce steps than \Hma, the size of the intermediate data (and hence the communication) can become prohibitively large for sparse graphs with a large number of components. We now present \Hm, a variation on \Ha, that has the (asymptotic) communication cost of  \Hma while completing in just $O(\log d)$ map-reduce steps.

 In \Hm, the hash function $\h$ computes the smallest node in the cluster $\TC(v)$ and sends two kinds of messages. The entire cluster $\TC(v)$ is sent to the smallest node $v_{\min}$, and the smallest node is sent to all the other nodes in the cluster; i.e., the set of messages is $\{(\TC(v), v_{\min})\} \cup \{(\{v_{\min}\}, u) \mid u \neq v_{\min} \in \TC(v)\}$.

 The local aggregation function $\Md$ works exactly like in \Ha: $\TC(v)$ is the union of all the nodes appearing in the received messages. However, unlike \Ha, at the end of the algorithm all nodes are not guaranteed to contain in $\TC(v)$ the connected component they are part of. In fact, we can show that, the smallest node in a connected component contains all the nodes in that components, while for other nodes $\TC(v) = \{v_{\min}\}$. Hence, \export outputs only those $\TC(v)$ such that $v$ is the smallest node in $\TC(v)$.

 \begin{lemma}\label{lemma:hm}
 At the end of algorithm \Hm, $\TC(v)$ satisfies the following property. If $v_{\min}$ is the smallest node of a connected component $C$, then $\TC(v_{\min}) = C$. For all other nodes $v$, $\TC(v) = \{v, v_{\min}\}$.
 \end{lemma}
 \begin{proof}(sketch)
 Any node $u$ connected to the smallest node in the component $v_{\min}$ is guaranteed to receive $v_{\min}$. As a result, in the next step, $u$ sends all its nodes to $v_{\min}$ and only $v_{\min}$ is sent to $u$. Since at some point of time all nodes know $v_{\min}$, every node $u$ sends its cluster to only $v_{\min}$ and thus $u$ does not get any other message other than $v_{\min}$.
 \end{proof}
 
We conjecture that this always finishes in $2 \log d$ steps with an expected communication cost (over all permutations of node ids) bounded by $O(\nnodes + \nedges)$ per iteration.  We can show examples of  graphs where the node ids are such that the communication cost could grow as large as $O(\nnodes^2)$ per iterations. Hence, \Hm randomly assigns ids to nodes in the graph -- thus making it a randomized algorithm.
%We can bound the communication cost by $O(\nnodes + \nedges)$ with high probability, by first randomizing the node ids in a preprocessing map step. This makes \Hm a randomized algorithm.


\subsection{\Hcm Algorithm}

In \Hcm, each node $v$ maintains a set $\core_v \subseteq \TC_v$  of all nodes that have $v$ as the minimum. Initially, $\core_v = v$. In each iteration, hash function $\h$ computes the smallest node in the cluster $\TC(v)$ and sends two kinds of messages. The set $\core(v)$ is sent to the smallest node $v_{\min}$, and the smallest node is sent to all nodes in $\core_v$; i.e., the set of messages is $\{(\core_v, v_{\min})\} \cup \{(\{v_{\min}\}, u) \mid u \neq v_{\min} \in \core_v\}$.

We now analyze the performance of an algorithm, called \alternating, that does an iteration of  \Hma, followed by another iteration of \Hma, and then a iteration of \Hcm, and keeps on repeating these three iterations until convergence.


 \begin{theorem}[\Hcm]
 Algorithm \alternating correctly computes the connected components of  $G = (V,E)$ in expected $3\log{n}$ map-reduce iterations. Here expectation is over the random choices of the node ordering. The algorithm takes $2(\nnodes + \nedges)$ complexity per iteration in the worst-case.
 \end{theorem}
 \begin{proof}(sketch)
 Correctness follows from Lemma~\ref{lemma:hm}.

 \eat{We first show that after every iteration of \Hcm clusters are reflexive, i.e. if a node $v' \in TC_v$, then the node $v \in TC_{v'}$. This follows trivially since either $v$ is the minimum and $v' in \core(v)$ or the other way around. In either case, $v' \in TC_v$ and $v \in TC_{v'}$.
 }

After $k$ iterations, denote $M_k =  \{ min(\TC_v) : v \in V \}$ the set of nodes that appear as minimum on some node. For a minimum node $m \in M_k$, denote $core_k(m)$ the set of all nodes $v$ for which $m = min(\TC_v)$.  Obviously $\cup_{m \in M_k} core_k(m) = V$ and  for any $m,m' \in M_k$, $core_k(m) \cap core_k(m') = \emptyset$.

Consider the graph $G_{M_k}$ with nodes as $M_k$ and an edge between $m \in M_k$ to $m' \in M_k$ if there exists $v \in core_k(m)$ and $v' \in  core_k(m')$ such that $v,v'$ are neighbors in the input graph $G$.  If a node $m$ has no outgoing edges in $G_{M_k}$, then $core_k(m)$ forms a connected component in $G$ disconnected from  other components, this is because, then for all $v' \notin core_k(m)$,  there exists no edge to $v \in core_k(m)$.

\eat{ If a node $m$ has no outgoing edges in $G_{M_k}$, then $core_k{m}$ forms a connected component in $G$ disconnected from  other components. This is because, since $m$ has not outgoing edge in $G_{M_k}$, for all $v' \notin core_k(m)$, we know that $v' \notin \TC_v$ for all $v \in core_k(m)$. Since if $v' \notin \TC_v$, then by reflexivity shown above, we know that $v \notin \TC_{v'}$, hence for all $v in Cl_k(m)$ and $v' \notin \TC_v$, $v \notin TC_{v'}$. This means that no $v \in Cl_k(m)$ can get any $v' \notin Cl_k(m)$ even in iteration $k+1$. So even in the next iteration $Cl_k(m)$ remains the same, and hence $Cl_k(m)$ is a component in $G$ disconnected from other components.
}

We can safely ignore such sets $core_k(m)$. Let $MC_k$ be the set of nodes in $G_{M_k}$ that have at least one outgoing edge. Also if $m \in MC_k$ has an edge to $m' < m$ in $G_{M_k}$, then $m$ will no longer be the minimum of nodes $v \in core_k(m)$ after $3$ iterations. This is because there exist nodes $v \in \core_k(m)$ and $v' \in \core_k(m')$, such that $v$ and $v'$ are neighbors in $G$. Hence in the first iteration of \Hma, $v'$ will send $m'$ to $v$. In the second iteration of \Hma, $v$ will send $m'$ to $m$. Hence finally $m$ will get $m'$, and in the iteration of \Hcm, $m$ will send $\core_k(m)$ to $m'$.

If $|MC_k| = l$, W.L.O.G, we can assume that they are labeled $1$, $2$, \ldots, $l$ (since only relative ordering between them matters anyway).  For any core, $\core_k(m)$, the probability that it its min $m' \in (l/2,l]$ after 3 more iterations is $1/4$. This is because  that happens only when $m \in [(l/2,l)$ and all its neighbors $m' in G_{M_k}$ are also in $(l/2,l]$. Since there exist at least one neighbor $m'$, the probability of $m' \in (l/2,l]$ is at most $1/2$. Hence the probability of any node $v$ having a min $m' \in (l/2,l]$ after 3 more iterations is 1/4.

Now since no core, $\core_k(m)$, ever get splits in subsequent iterations, the expected number of cores is 3l/4 after 3 more iterations. Hence in three iterations of \alternating, the expected number of cores reduces  from $l$ to $3l/4$, and therefore it will terminate in expected $3\log{n}$ time.


The proof of $2(\nnodes + \nedges)$ complexity per iteration in the worst-case is trivial since total size of clusters is $\sum_{v} \core_v = 2 (\nnodes)$.\end{proof}


 \subsection{Discussion: Comparing the different algorithms}
 While \Hm has the best asymptotic complexity compared to \Hma and \Ha, no algorithm dominates other algorithms in all respects. First, while \Ha has significantly higher communication cost than \Hm, it computes the connected components in {\em exactly} $\log d$ steps; on the contrary, \Hm takes twice the number of steps on most graphs.  Next while \Hm (and \Ha) takes significantly smaller number of steps than \Hma, note that until the export step, each node only maintains its neighbors and the smallest node it knows of. However, in \Hm and \Ha, at least one node contains the entire cluster -- which might be undesirable if the number of nodes in a component is very large. Hence, our recommendation is that for very sparse graphs with large diameter, one should use \Ha; for graphs with large diameter one should use  \Hm; and for graphs with small diameter one should use \Hma. 

==> changes.tex <==
\eat{Planned changes:

1. Address why map-reduce is required. Twitter graph has 142M edges, which roughly corresponds 2.5G, assuming 8 bytes per id. 
   Demonstrate that connected components on a single laptop does not work well for such graphs.

2. Use dense graphs in addition to the sparse ones.

Changes done:

}

\onecolumn

\begin{center}
 {\huge{\bf Changes Done}}\\ \vspace{0.1in}
\end{center}

We thank the reviewers for their time and invaluable comments. For the
revision, we focused on presentation changes to make the paper
readable. Some of the comments by reviewers greatly helped us to do
that. Below we list the changes that we've made.

\paragraph{Introduction (Sec. 1):} In the introduction, we changed the
paragraph describing secondary sorting. We motivated the reason why
this is required and why this helps.

\paragraph{Related Work (Sec. 2):} We added a reference to the work by
``T. Seidl, B. Boden, S. Fries: CC-MR – Finding Connected Components
in Huge Graphs with MapReduce. In ECML/PKDD, 2012''. 

\paragraph{Algorithms (Sec. 3):} This is the section where we made most of the
presentation changes. This is the most important technical section of
the paper, and the section which had most concerns from the
reviewers.
 
\begin{enumerate}
\item We removed references to explicit machines and just used standard notation
of keys and values in map-reduce. This greatly simplifies the
presentation. We thank reviewer 3 for this suggestion.

\item We added/clarified examples for hash-to-min, hash-to-all, and hash-greater-to-min. We thank reviewer 2 for this suggestion.

\item We included more details in the proof for this section, since this is
the most important technical section. All the proof sketches have been
replaced by full proofs. A couple of proofs still had to be omitted
because of space limitations. 

\item The ommited proofs appear in the full version of the paper~\cite{fullversion}.

\end{enumerate}

\paragraph{Scaling the Hash-to-min Algorithm (Sec. 4):} We clarify a concern of reviewer 1 (weak point 2) by adding this sentence: "Note that this increases the number of rounds by at most 2, as after load-balanced \Hm converges, we use the standard \Hm." 

\paragraph {Clustering (Sec. 5):} We removed detailed proofs from
the clustering section to make room for examples and detailed proofs
in Section 3. The detailed proofs for this section are also available in the full
version~\cite{fullversion}.


==> clustering/extensions.tex <==
\section{Extensions}
\label{extensions}

\input{cc/hybrid}

\eat{
\subsection{Extensions to Distributed Inference}
\label{sec:distributed-inference}
Junction-tree inference is the procedure to compute the joint probability distribution of any set $Q$ of variables in a junction-tree. The joint probability distribution is a function $Pr$ mapping subsets $S \subseteq Q$ to reals such that $$\sum_{S \subseteq Q} Pr(S) = 1$$

We can extend our framework for distributed clustering to the problem of junction tree inference as follows. We represent each variable of the junction tree using a node in $V$. The junction-tree $J$ can then be thought of as a clustering $\C_J$ of $V$ along with the joint probability distribution $Pr$ of over all $C \in \C$. Next we mention how to define the distance $d$ between two clusters used in our clustering framework:  $d(C_1,C_2) = 0$ if they overlap, i.e. $C_1 \cap C_2 \neq \emptyset$ and $1$ if they do not, i.e. $C_1 \cap C_2 = \emptyset$.

With this definition of cluster distance, we can again use Algorithm 1 to do junction-tree inference in map-reduce. Initialization for inference is different than that described in the framework above. We initialize the clustering not as singleton clusters this time, but as $\C_J$ corresponding to the junction tree $J$.  For the hashing function, we use \Ha, which is guaranteed to map two overlapping clusters to some common reducer.

In the reducer, we use a special merging function $\Md$, which merges incoming clusters $C_1,\ldots,C_k$ to computes $C = \cup_i C_i$. It then computes the joint probability distribution of $C$ using the distributions of individual $C_i$'s. Finally, it projects out variables from $C$ not in $Q$. These are done in the standard way by the equations below. $$\forall S \subseteq C_1 \cup C_2, Pr(S)  = Pr(S \cap C_1)Pr(S \cap C_2)/Pr(S \cap S_1 \cap S_2)$$ $$\forall S \subseteq (C_1 \cup C_2 )\cap Q, Pr(S)  =  \sum_{S'  \subseteq C_1 \cup C_2, S' \cap Q = S} Pr(S)$$

We can show that the above algorithm finishes in $O(\log{d})$ map-reduce rounds where $d$ is the diameter of the junction tree. This is significantly lower that $O(d)$ rounds required in previous work~\cite{pegasus}. The communication per round is  $O(n\nnodes + n^2)$. Since $n$ is usually small in junction trees (especially, for graphical models with low tree width), the communication cost is reasonably small.
}



==> clustering/generic.tex <==
\section{Generic Distributed Algorithm}
\label{sec:generic}

In this section we formally define our generic approach to distributed clustering and inference. In Section~\ref{subsec:centralized} we start by formalizing a centralized framework that captures many clustering and inference algorithms; Section~\ref{subsec:instantiations} instantiates this framework some of the popular clustering algorithms. Then, in Section~\ref{subsec:distributed} we introduce the main building blocks for distributed clustering, along with illustrative examples. Details of these building blocks are the subject of subsequent sections.

\subsection{Generic Centralized Framework}
\label{subsec:centralized}

\begin{definition}[Clustering]
A clustering of a set $E = \{e_1, \ldots, e_n\}$ of entities is a set $\C=\{C_1, \ldots, C_k\}$ of clusters such that $C_i \subseteq E$ for all $i \in \{1,2,\ldots,k]$. % $S = \bigcup_{i=1..k} C_i$. %, (b) if $i\neq j$, $S_i \cap S_j = \emptyset$.
\end{definition}

We describe below a simple yet powerful generic framework that captures many clustering and inference algorithms. The framework essentially works bottom up,  using a {\em distance function} between clusters to choose a pair of clusters,  a {\em merging predicate} to decide whether the pair should be merged, a {\em merging function} that combines the pair in some way, and finally a {\em stopping criterion} to decide whether a cluster is ready to be output.

\begin{definition}[Distance Function]
A distance function $\D:2^{E}\times 2^{E}\rightarrow [0,1]$ is a function that returns a {\em distance} in $[0,1]$ for any pair of clusters of $E$.
\end{definition}

\begin{definition}[Merging Predicate]
A merging predicate $\Pred: 2^{E}\times 2^{E}\rightarrow \{0,1\}$ returns, for any pair of clusters of $E$,  either $1$ or $0$, indicating whether the clusters should be merged or not.
\end{definition}

\begin{definition}[Merging Function]
A merging function $\Merge: 2^{E}\times 2^{E}\rightarrow 2^{E}$ returns, for any pair of clusters of $E$, a single cluster.
\end{definition}

\begin{definition}[Stopping Criterion]
A stopping criterion is defined by a predicate $\Stop(\C)$ that,  for any clustering $\C$ of  $E$, returns $1$ or $0$ indicating whether to stop the clustering process.
\end{definition}

Any centralized algorithm $\A(\D,\Pred,\Merge,\Stop)$ proceeds as in Algorithm~\ref{algo:central}: It first initializes a candidate clustering $\C$ as singleton element sets. Then it seeks to combine candidate clusters by repeatedly picking a pair of clusters from $\C$ that  are closest according to distance function $\D$ and allowed to merge according to $\Pred$, and replaces the original pair from $\C$ by the merged cluster. It then checks whether to stop the clustering process using the $\Stop$ criterion. Once stopped, it returns the clustering $\C$.
% For our presentation in Section~\ref{sec:hashing}--\ref{sec:results} we shall assume a simple ``no stop'' condition, i.e., clusters are formed until no more merges can happen. We shall then address the subtleties in handling non-trivial stopping criteria in Section~\ref{sec:stopping}.

%For the rest of the paper, we restrict our attention to a standard stopping criterion for agglomerative clustering algorithms: . We note that other commonly applied stopping criterion (such as threshold on similarity, or until no merges can happen) can be handled by our approach in an identical fashion.


\begin{algorithm}[t]
\caption{Generic Framework $\A(\D,\Pred,\Merge,\Stop)$}
\begin{algorithmic}[1]
\STATE {\bf Input:} Set $E$ of entities, distance function $\D$, merging predicate $\Pred$, merging function $\Merge$, stopping criterion $\Stop$
\STATE {\bf Output:} A clustering $\C_{out}$ of $E$ %such that $E = \bigcup_{C\in \C} C$.
\STATE Initialize candidate clustering $\C = \{\{e\} | e\in E\}$;
 \WHILE{$\C$ changes}
 \STATE Find the closest mergable pair of clusters $C_1,C_2$ in $\C$~(according to $\D$ and $\Pred$);
 \STATE Update $\C = \C -\{C_1,C_2\} \cup \{ \Merge(C_1,C_2) \}$;
\IF{$\Stop(\C)=1$}
  \STATE break;
\ENDIF
\ENDWHILE
\STATE Return $\C$
\end{algorithmic}
\label{algo:central}
\end{algorithm}


\subsection{Instantiations of the Framework}
\label{subsec:instantiations}

Next we explain how the above framework can be instantiated to do agglomerative and correlation clustering as well as junction-tree inference.

\paragraph{Agglomerative Clustering} is an iterative technique that starts with singleton clusters and in each iteration greedily merges the two closest clusters to form a single larger cluster.  We now explain how $\D$, $\Pred$, $\Merge$, $\Stop$  can be defined to obtain an agglomerative clustering algorithm.

For distance function $\D$, many variations exist among different algorithms. Usually any arbitrary distance function $d$ between pairs of entities is assumed to be known. Then the distance $\D$ between clusters is expressed using distance between individual entities in the clusters.  For single-linkage agglomerative clustering, $\D(C_1,C_2)$ is the distance of closest entities, $\min_{e_i \in C_1, e_j \in C_2} d(e_i,e_j)$. For complete-linkage, $\D(C_1,C_2)$ is the distance of the two farthest entities, while for average-linkage,  $\D(C_1,C_2)$ is the average distance between pairs of entities in the two clusters. For merging predicate $\Pred$, always returning $1$ suffices. For merging function, simple union operation suffices, so $\Merge(C_1,C_2) = C_1 \cup C_2$.

For stopping criterion $\Stop$, there are a couple of possibilities that are used often. Distance-threshold based algorithms stop processing a clusters if its closest cluster has a distance greater than a threshold. On the other hand, size-threshold based algorithms stop if the cluster's size is greater than a threshold. In general, any $\Stop$ can be used in our framework, as long as it is monotonic, i.e. $\Stop(C)=0 \Rightarrow \Stop(C')=0$ for any $C \subset C'$.

\paragraph{Correlation Clustering} is a clustering technique that uses both positive and negative edges between entities to form clusters. A (negative) positive edge between a pair of entity means they are (not) likely to lie in the same cluster. Formally, this is achieved by finding clusters that maximize a linear combination of inter-cluster positive and intra-cluster negative edges. Many algorithms have been proposed for different kinds of edges (soft, hard, with/without weights). Here we focus on the algorithm proposed in~\cite{dedupalog} that handles both soft (but having unit weight) and hard edges (having infinite weights).  The algorithm chooses a random permutation of all the edges and `hardens' edges in that order. Hardening a positive edge between two entities means that the clusters containing the two entities should be merged unless there exists an already hardened negative edge between two entities of the clusters. Hardening a negative edge means that the clusters should never be merged in the future.

We now explain how $\D$, $\Pred$, $\Merge$, $\Stop$  can be defined to obtain the above correlation clustering algorithm. For distance function $\D$, we first randomly generate a distance function $d$ between pairs of entities. This is done by choosing a random number as the distance for every pair of entities. Then the distance $\D$ between clusters is the distance of the closest entities such that a positive edge exists between them. More formally,  $\D(C_1,C_2) = \min_{e_i \in C_1, e_j \in C_2, (e_i,e_j)=+} d(e_i,e_j)$.

For merging predicate $\Pred$, we merge two clusters $C_1,C_2$ iff the first 'hardened' edge going across them is positive. This happens when the minimum distance among pairs of entities in the two clusters having a positive edge is smaller than that for a negative edge. More formally, the following should hold $$ \min_{e_i \in C_1, e_j \in C_2, (e_i,e_j)=+} d(e_i,e_j) <  \min_{e_i \in C_1, e_j \in C_2, (e_i,e_j)=-} d(e_i,e_j)$$
For merging function $\Merge$, again a simple union operation suffices, so $\Merge(C_1,C_2) = C_1 \cup C_2$. For stopping criterion $\Stop$, returning always $0$ suffices.

\paragraph{Junction-tree inference} is the procedure to compute the joint probability distribution of any set $Q$ of variables in a junction-tree. The joint probability distribution is a function $Pr$ mapping subsets $S \subseteq Q$ to reals such that $\sum_{S \subseteq Q} Pr(S) = 1$. To adapt such algorithms in the framework above, we represent each variable of the junction tree assume by an entity in $E$. The junction-tree $J$ can then be thought of as a clustering $\C_J$ of $E$ along with the joint probability distribution $Pr$ of all $C \in \C$.

Initialization for inference is different than that described in the framework above. We initialize the clustering not as singleton clusters this time, but as $\C_J$ corresponding to the junction tree $J$. Next we mention how to set $\D$, $\Pred$, and $\Merge$ to do inference.

For distance function $\D$, $\D(C_1,C_2) = 0$ if $C_1 \cap C_2 \neq \{\}$ and $1$ if $C_1 \cap C_2 = \{\}$. For merging predicate $\Pred$, $\Pred(C_1,C_2) = 1$ if $C_1 \cup C_2 \cap Q$ and $0$ otherwise. For merging function $\Merge$,  we first find the joint probability distribution of $C_1 \cup C_2$ and then  project out any variable in $C_1 \cup C_2$ not in $Q$. These are done in the standard way by the equations below. $$\forall S \subseteq C_1 \cup C_2, Pr(S)  = Pr(S \cap C_1)Pr(S \cap C_2)/Pr(S \cap S_1 \cap S_2)$$ $$\forall S \subseteq (C_1 \cup C_2 )\cap Q, Pr(S)  =  \sum_{S'  \subseteq C_1 \cup C_2, S' \cap Q = S} Pr(S)$$


\subsection{Distributed Approach}
\label{subsec:distributed}

Next we present our generic distributed algorithm. Algorithm~\ref{algo:distributed} shows the building blocks of the distributed algorithm. It is run on a set of machines $\{v_1,\ldots,v_{K}\}$, and consists of series of map-reduce iterations. Each entity $e \in E$ has a reducer that we denote as $\machine{e}$. In the map task, we hash clusters to sets of machines. For this we use a hashing function $\h$, that takes a single cluster $C$ and returns a set of cluster-machine pairs $\{(C_i, v_j)\}$ where $1\leq j \leq K$, signifying that cluster $C_i$ should be sent to machine $v_j$.

In the reduce task, we do two things on each machine: (i) Locally run centralized algorithm $\A$ to (re-)cluster the set of elements on the machine, and (ii) check whether the machine should be stopped, by checking whether clustering remains unchanged in the iteration, and also checking for the given stopping condition. The map-reduce iterations continue as long as some machine is active (i.e. not stopped).

 \eat{The core data structure maintained at every machine is a {\em forest} of elements to be clustered:

\begin{definition}[Forest]
Given a set of entities $E = \{e_1, \ldots, e_n\}$ of entities, a forest $F$ over $E$ is defined by a set of node-disjoint trees over a subset of the entities.
\end{definition}

\noindent Intuitively, the forest keeps track of each partial cluster, and also the history of how the cluster was formed. We shall see later that the history may be used to retrace incorrect merges. Such incorrect merges may happen due to local computation that only operates on a subset of the total set of entities.
}

\eat{\begin{definition}[Distributed Clustering]
A distributed clustering algorithm $\DC_\A(\h,\Sd)$ is run on $K$ machines and has  three main steps:

(1)

(2) local-transformation function $\M$ that takes as input a set $\{C_1, C_2, \ldots, ..., \}$ and returns a single forest $C$

(3) stopping-condition check:  to distributedly check for stopping criterion $\Stop$.
\end{definition}
}

\noindent Note that Algorithm~\ref{algo:distributed} doesn't specify how the hash function $\h$ and the stopping condition $\Sd$. We shall describe them in Sec.~\ref{sec:hashing} and Sec.~\ref{sec:stopping}, respectively. %As described earlier, we start by restricting our attention to a trivial stopping condition that only terminates the algorithm when all possible merges have finished. In practice, there are a wide variety of stopping conditions that can be handled by our distributed approach---including those of most popular clustering algorithms---and


\begin{algorithm}[t]
\caption{Distributed clustering algorithm $\DC_\A(\h,\Sd)$}
\begin{algorithmic}[1]
\STATE {\bf Input:} Set $E$ of entities, hashing function $\h$,  local transformation $\Md$, stopping criterion $\Sd$.
\STATE Initialize candidate clustering $\C = \{\{e\} | e \in E\}$.
\WHILE{some machine is active}
\STATE {\bf Map:} For $C \in \C$, compute $\h(C)$, and for each $(C_i, v_i) \in \h(C)$, send $C_i$ to machine $v_i$.
\STATE {\bf Reduce on machine $\machine{e}$:}
\STATE  Let $\C_{in}(e)$ be set of all clusters sent to machine $\machine{e}$.
\STATE Compute $\A$ on  $\C_{in}(e)$ to get new clustering $\C_{out}(e)$.
 \IF{$\Sd(\C_{out}(e))=1$ or $\C_{out}(e) = \C_{in}(e)$}
   \STATE Output $\C_{out}(e)$, and stop machine $\machine{e}$.
\ENDIF
\ENDWHILE
\end{algorithmic}
\label{algo:distributed}
\end{algorithm}


\eat{
\begin{algorithm}[t]
\caption{Distributed clustering algorithm $\DC_\A(\h,\Sd)$}
\begin{algorithmic}[1]
\STATE {\bf Input:} Set $E$ of entities, hashing function $\h$,  local transformation $\Md$, stopping criterion $\Sd$.
\STATE Initialize candidate clustering $\C = \{\{e\} | e \in E\}$ and send clustering $\C_{in}(e) = \{\{e\}\}$ to machine $\machine{e}$.
\WHILE{$\C_{in}(e)$ changes on any machine $\machine{e}$, in $\machine{e}$}
\STATE  Compute $\A$ on all clusters in $\C_{in}(e)$ to get a new clustering $\C_{out}(e)$.
\IF{$\Sd(\C_{out}(e))=1$}
 \STATE Output $\C_{out}(e)$ and stop machine $\machine{e}$.
\ELSE
\STATE For all clusters $C_{out} \in \C_{out}(e)$, compute $\h(C_{out})$ and for each $(C, v) \in \h(C_{out})$, send $C$ to machine $v$.
\STATE Recompute $\C_{in}(e)$ equal to set of all clusters sent to machine $\machine{e}$.
\ENDIF
\ENDWHILE
\end{algorithmic}
\label{algo:distributed}
\end{algorithm}
}


\eat{
\begin{algorithm}[t]
\caption{Distributed clustering algorithm $\DC(\h,\M,\Pred)$}
\begin{algorithmic}[1]
\STATE {\bf Input:} Set $E$ of entities, hashing function $\h$,  local transformation $\M$, stopping criterion $\Pred$, maximum number of candidates $K$.
\STATE {\bf Output:} A clustering $\C \subseteq 2^E$ such that $E = \bigcup_{C\in \C} C$.
\STATE Initialize current forest set  $\F = \{\{F_e\} | e\in E\}$; {\em change}$=0$
\WHILE{$F_e \in \F$\ changes on any machine $\machine{e}$}
\STATE In machine $\machine{e}$: Compute $\h{F_e}$. For each $(F_i, v_i) \in \h(F_e)$, send $F_i$ to machine $v_i$.
\STATE In machine $\machine{e}$: Compute $M$ on all Forests in the machine to get $F'_e$ .
\STATE Check for stopping condition.
\STATE $\F=\F'$; {\bf break;}
\ENDWHILE
\end{algorithmic}
\label{algo:central}
\end{algorithm}
} 

==> clustering/hashing.tex <==
\section{Hashing Schemes}
\label{sec:hashing}


%Given a distance function $\D$, we first define the notion of distance graph.

%\begin{definition} Let $\D$ be a distance function over pairs of clusters of entities in $E$. The distance graph $G_{\D}$ for $\D$ is a weighted graph with nodes as entities in $E$ and edges between two entities $(e_1,e_2)$ with weight $\D(\{e_1\},\{e_2\}).
%\end{definition}

This section describes the hashing step of Algorithm~\ref{algo:distributed}. Recall, a hashing scheme is a function that takes as input a cluster $C$ and returns a set of cluster-machines pairs, representing what information is sent to which machine. Recall that we have a reducer machines for each entity $e$ in $E$ and denote it by $\machine{e}$. Our hashing schemes also require a total ordering over the elements in $E$, and we denote for any cluster $C$, $min(C)$ the minimum element according to this ordering among entities in $C$.

For an entity $e \in E$, denote $\nD{e}{\D}$ the set of all entities $e'$ that have a finite distance $\D(\{e\},\{e'\})$. When $\D$ is clear from context, we denote the set simply as $\n{e}$. Also denote $\n{C}$ for a cluster of entities $C$ the set of all entities in the union of $\n{e}$ for $e \in C$. Denote $\nn{e}$ the set of all entities in $\n{e}$ that have the smallest distance to $e$. Finally denote $\nn{C}$ the set of all entities $e$ in $\n{C}$ that have the smallest distance $\D(\{e\},C)$.

%We say a hashing scheme is lossless if $F_1 \cup \ldots \cup F_K = F$ and only consider lossless hashing schemes. 

We describe three hashing functions: \Ha\ ($\ha$ for short), \Hm\ ($\hm$ for short), \Hs($\hn$ for short) in this section. We also give a brief example to illustrate the difference between these hashing schemes.

\paragraph{\Ha\ Scheme}  Let $C$ be a cluster of entities.  \Ha\ is a simple hashing scheme, defined formally as $\ha(C) = \{(C, \machine{e}) | e \in C \cup \n{C}\}$, in which we send the entire cluster to machines corresponding to each of the entities in the cluster and their neighbors.

\paragraph{\Hm\ Scheme}  Recall that \Ha\ scheme sends the cluster $C$ to all machines $\machine{e} \in C$. The hashing scheme \Hm\ sends the entire cluster $C$ to only one machine, which corresponds to the minimum element $m = min(C)$. For all elements $e \in C \cup \n{C}$ other than $m$, the hashing scheme sends to $\machine{e}$, the cluster $\{e,m\}$.  Formally, $\hm$ is defined as:  $\hm(C) = \{(C,m\} \cup \{(\{m,e\},e) | e \in C \cup \n{C} - \{m\}\} $.

\paragraph{\Hn\ Scheme}  The hashing scheme \Hn\ sends the entire cluster $C$ to none of the machines. Again denoting $m=min(C)$, for all elements $e \in C \cup \nn{C}$, then the hashing scheme sends to $\machine{e}$, the cluster $\{e,m\}$.  Formally, $\hn$ is defined as:  $\hn(C) = \{ \{(\{m,e\},e) | e \in C \cup \nn{C}\} $.


\subsection{Example}
\label{subsec:h-ex}

The main difference between the \Ha\ scheme and the \Hm\ scheme is that \Ha\ transmits much more data in the hash step, which may lead to a prohibitive communication complexity, and large intermediate data size if $F$ is large. On the other hand, \Hm\ transmits much less data. Yet, surprisingly, In section~\ref{sec:results} we give theoretical results that show that \Hm\ significantly lowers the communication complexity for a constant-factor increase in the number of map-reduce steps. We also experimentally compare the two schemes on multiple datasets in Section~\ref{sec:experiments}. Next we give a short example to illustrate how the two hashing schemes work.






==> clustering/hashing_v2.tex <==
\subsection{Hashing}
\label{sec:slc_hash}
We use two hashing schemes for \slc -- \Ha and \Hm. In \Ha, we send the entire cluster $\TC(v)$ to each node $u \in \TC(v)$ as well as all the neighbors of $u$.  

==> clustering/intro.tex <==
\section{Introduction}
\label{sec:intro}

Clustering~\cite{} is one of the most studied problems in Computer Science, with wide-ranging applications in entity de-duplication,  social networking, inference in graphical models, topical or structural  clustering of web-pages, spam detection, and areas outside Computer Science~\cite{}. While each application may use a different clustering algorithm, a common feature across many of these applications is that they  deal with an extremely large amount of data, rendering centralized (single-machine) clustering impractical. %(In Section~\ref{sec:motivation}, we shall see concrete examples of clustering along with the data size they operate on.) 
This paper addresses the challenge of performing {\em distributed clustering}, in a cloud environment. 


In contrast, we present the first {\em generic} distributed clustering framework that applies to a large class of clustering algorithms, namely, transitive closure clustering, single-linkage and non-single-linkage agglomerative clustering, correlation clustering, and clustering for distributed inference. We develop techniques for distributed clustering using map-reduce. Intuitively. 
We broadly consider the following four types of clustering algorithms:

\begin{enumerate}
\item {\bf Agglomerative clustering:} Agglomerative clustering algorithms build clusters in a {\em bottom-up} fashion, starting with individual elements in singleton clusters. Thereafter, based on a predefined distance metric, the closest pairs of clusters are merged, until a stopping criterion is reached. We consider {\em single-linkage} agglomerative cluster, where the distance between two clusters is the edge distance of the closest pair of elements, as well as {\em non-single linkage} clustering, which uses any arbitrary distance metric.

\eat{Our mapreduce will include a map phase which uses LSH to hash nodes to preserve the distance metric. It then divides the space of LSH into intervals and maps all hashes in the interval together. Then the reduce step will merge the closest pair. We might have to unmerge things if we later find a closer solution. Exact details need to be worked out.}

\item {\bf Connected-components clustering:} Given a graph with un-weghted edges, we are simply interested in the connected components of the graph. 

\item {\bf Correlation clustering:} There are positively/negatively weighted edges. Goal is to find clusterings that have large positive edges within clusters and small negative edges that cross clusters. Depending on the weights allowed, there are centralized algorithms that achieve good approximation ratios. Note that correlation clustering is a generalization of connected components clustering.
\eat{This is a strict generalization of transitive closure Ñ for which we have two algos that I call: hash-to-all and hash-to-min. Can we obtain a mapreduce implementation for the general problem?}

\item {\bf Clustering for inference in graphical models:} Finally, we also consider performing inference in large graphical networks, which requires a localized version of clustering: the graph is constructed with random variables as nodes, and edges depicting correlations between variables. Inference involves traversing connected components in the graphical network in a fashion such that all intermediate clusters are connected~\cite{}.

\end{enumerate}


The two important metrics in comparing distributed algorithms for clustering are: {\em number of map-reduce steps} and {\em communication cost}. The number of map-reduce steps is a measure of the latency of the algorithm, and the communication cost determines the memory requirement on mappers and reducers. We shall see that our general framework for clustering improves upon the best known previous algorithms, both in terms of number of map-reduce steps and in terms of the communication cost. A particularly salient feature of our framework is that it works very efficiently on graphs with large diameter, while most previous approaches have been tailored towards graphs with low diameter (since the web graph has a low diameter). We note that several applications such as traffic networks~\cite{}, social graphs~\cite{}, and graphical models~\cite{}  involved clustering in graphs with high diameters.


\begin{table*}[t]
\centering
\begin{tabular}{ |c|c|c|c|c| }
  \hline 
Technique &  Hashing & Merging &  \multicolumn{2}{|c|}{Complexity}  \\ 
  \cline{4-5}
    &&& of MR Steps & Communication per MR step \\
  \hline
\multirow{2}{*}{Transitive Closure} & $\ha$ & $\M$ & $O(\log{d})$ &  $  O(n^2N  + M)$\\
\cline{2-5}
  & $\hm$ & $\M$ & $O(\log{d})$  &  $  O(N  + M)$\\
  \hline  
\multirow{2}{*}{\parbox[c]{4cm}{\centering Single-linkage \\ Agglomerative Clustering}} & $\ha$ & $\M$ & $O(\log{n})$ &  $  O(n^2N  + M)$\\
\cline{2-5}
  & $\hm$ & $\M$ & $O(\log{n})$  &  $  O(N  + M)$\\
  \hline  
  \parbox[c]{4cm}{\centering Other-linkage \\ Agglomerative Clustering} & $\ha$ & $\M$ & $O(\log{n})$ &  $  O(n^2N  + M)$\\
  \hline  
\multirow{2}{*}{Correlation Clustering} & $\ha$ & $\M$ & $O(n)$ &  $  O(n^2N  + M)$\\
\cline{2-5}
  & $\hm$ & $\M$ & $O(n)$  &  $  O(N  + M)$\\
  \hline  
Distributed Inference & $\ha$ & $\M$ & $O(\log{d})$ &  $  O(n^2N  + M)$\\
  \hline  
\end{tabular}

\caption{Techniques supported by our distributed framework and their complexity. }
\end{table*}


\begin{table}[t]
\begin{tabular}{ |c|c| }
  \hline 
 Symbol & Semantics \\
 \hline
 N & \# of nodes in the graph \\
 M & \# of edges in the graph \\
 n & \# of nodes in the largest cluster \\
 d & longest diameter of any cluster \\
 \hline  
\end{tabular}
\caption{Notation}
\end{table}


\subsection{Contributions and Outline}

The main contributions of this paper are as follows:

\begin{enumerate}

\item We propose a generic map-reduce framework for graph clustering algorithms, with a map phase that corresponds to hashing clusters to appropriate machines, and reduce phase performing local clustering. (Section~\ref{sec:generic})
\item Our generic clustering approach is instantiated with specific hashing, local computation, and stopping criterion. We enumerate these three steps for a variety of clustering algorithms in Sections~\ref{sec:hashing},~\ref{sec:local}, and~\ref{sec:stopping} respectively.
\item We theoretically analyze our distributed clustering algorithms, and present complexity results in Section~\ref{sec:results}. We show that our algorithms significantly beat previous distributed clustering algorithms in terms of number of map-reduce steps and communication cost.
\item We present detailed experimental results evaluating our clustering algorithms and compare them with previously proposed algorithms on multiple real-world datasets. (Section~\ref{sec:experiments})
\end{enumerate}

Related work is presented in Section~\ref{sec:relatedwork}, and we conclude with future work in Section~\ref{sec:conclusions}.



==> clustering/local.tex <==
\section{Local Computation}

In this section, we describe the local computation step in our distributed approach. Recall from Section~\ref{sec:generic}, the local computation step proceeds at each reducer node as follows: Each node receives a set of clusters and returns a single cluster as output. Intuitively, the single cluster is obtained by locally executing the centralized clustering algorithm. More formally given a centralized algorithm $\A(\D,\Pred,\Merge,\Stop)$, and the set of clusters $\C_in{\machine{e}}$ on $\machine{e}$, the local computation runs $\A$ on $\C_{\machine{e}}$ to get clustering   

==> clustering/localTree.tex <==
\section{Local Computation}
\label{sec:local}

In this section, we describe the local computation step in our distributed approach. Recall from Section~\ref{sec:generic}, the local computation step proceeds at each reducer node as follows: Each node receives a set of forests and returns a single forest as output. Intuitively, the single forest is obtained by locally executing the centralized clustering algorithm, but keeping track of decisions made in the process (in the tree structure). 

First we intuitively describe the tree structure (Section~\ref{subsec:ts}), then describe an atomic tree merge step that is central to local computation (Section~\ref{subsec:tm}), and finally describe the merging of sets of forests in terms of atomic tree-merge steps (Section~\ref{subsec:fm}).

\subsection{Tree Structure}
\label{subsec:ts}

We start by describing the intuitive semantics of each tree in any forest. We use $T(N,E,L)$ to denote trees where $N$ is the set of all nodes in the tree, $E$ is the set of edges (inducing a tree), and $L\subseteq N$ is the set of leaf nodes in $T$. Each leaf node $l\in L$ corresponds to an entity being clustered, while each internal node $n\in N$ corresponds to a cluster. The set of entities in $n$ is given by all leaf descendants of $n$, denoted $\desc(n)$. In other words, a tree represents a sequence of merge steps resulting in the entire cluster, with each internal node giving an intermediate clustering. While our approach extends to any $n$-ary trees, for ease of discussion we restrict our attention to binary trees.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/tree.png}
\caption{\label{fig:tree}Example tree.}
\end{figure}

\begin{example}
Figure~\ref{fig:tree} shows an example of a simple tree in which entities $1$ and $2$ were merged, $3$ and $4$ were merged, and the resulting clusters were merged to create one final cluster of all four entities. (The merge of $1$ and $2$ may have happened either before or after $3$ and $4$.)
\end{example}

\subsection{Tree Merge}
\label{subsec:tm}

Next we describe the core idea behind the local computation step: merging a pair of trees to obtained a merged forest.

\begin{definition}[Tree Merge]
Given trees $T_1(N_1,E_1,L_1)$ and $T_2(N_2,E_2,L_2)$ and a pair of nodes $(n_1,n_2)$ to be merged, $n_i\in N_i$, a {\em tree merge} returns a forest $F=\treemerge(T_1,T_2,n_1,n_2)$ with leaf nodes $L_1\cup L_2$.
\end{definition}

\noindent Intuitively, a tree-merge is required to ``fix'' the sequence of merge operations encoded by each tree $T_1$ and $T_2$ independently: A merge of $n_1$ and $n_2$ in trees $T_1$ and $T_2$ results in a set of forests which is consistent with any ordering of merges in which all descendants of $n_i$ in $T_i$ (i.e, all merges that happened before the creation of $n_i$) are correct. However, all merges in each $T_i$ that happened using cluster $n_i$ were performed ``out of order'', so they need to be broken. 

The set of tree constituting the forest $F=\treemerge(T_1,T_2,n_1,n_2)$ are obtained as follows:

\begin{enumerate}
\item Initialize $F$ to an empty set of trees.

\item Construct a tree $T_{12}$ consisting of leaf nodes $\desc(n_1)\cup \desc(n_2)$ obtained by creating a new root node $n_{12}$ as the parent of subtrees of $T_1$ and $T_2$ rooted at $n_1$ and $n_2$ respectively.  Add $T_{12}$ to $F$.

\item For each $i=1,2$ construct trees from $T_i$ as follows:

\begin{enumerate}
\item Let $S_i$ be the (possibly empty) set of all ancestors of $n_i$ in $T_i$.

\item For each $s\in S_i$, find the child node $n^s_i\not \in (S_i\cup \{n_i\})$.

\item Add the subtree $T^s_i$ rooted at $n^s_i$ in $T_i$ to $F$

\end{enumerate}

\end{enumerate}

Intuitively, the resulting forest $F$ consists of all tree representing clustering that may have happened before the merge of $n_1$ and $n_2$.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figs/treemerge.png}
\caption{\label{fig:treemerge}Merge of trees $T1$ and $T2$ on nodes $n1$ and $n2$ to create a forest.}
\end{figure}

\begin{example}
Figure~\ref{fig:treemerge} shows an example merge.
\end{example}

\subsection{Forest Merge}
\label{subsec:fm}

Given a set ${\cal F}=\{F_1, \ldots, F_k\}$ of forests, a single forest is obtained by a sequence of tree-merge operations as follows: We find the closest pair nodes from any two forests (based on the distance measure used by the centralized algorithm), and merge the corresponding trees based on the tree-merge operation. We continue this process until the closest pair of nodes is farther than some pre-specified threshold or the merging criterion forbids the merge. (As a default case, all identical leaf nodes, and non-disjoint clusters from different trees will get merged given their default distance of $0$.) The pseudo-code for the forest merge algorithm appears in Algorithm~\ref{algo:fm}.






\begin{algorithm}[t]
\caption{Forest merge algorithm}
\begin{algorithmic}[1]
\STATE {\bf Input:} Set ${\cal F}=\{F_1, \ldots, F_k\}$ of forests.
\STATE {\bf Output:} Merged forest ${\cal F}^o$.
\STATE Let the set of all trees in any forest $F_i$ be ${\cal T}$. 
\STATE Initialize ${\cal F}^o = {\cal T}$.
\WHILE{stopping criterion not reached}
\STATE Find the pair of nodes $(n_1,n_2)$ from two distinct trees $n_i\in T_i$, where $T_i\in {\cal T}$ that have the next least distance.
\IF{Merge of $n_1,n_2$ allowed by the merging criterion}
\STATE ${\cal F}^o = {\cal F}^o-\{T_1,T_2\}\cup \treemerge(T_1,T_2,n_1,n_2)$
\ENDIF
\ENDWHILE
\end{algorithmic}
\label{algo:fm}
\end{algorithm}



















==> clustering/motivation.tex <==
\section{Motivating Examples}
\label{sec:motivation}

% Motivation
% Why does anyone want to do distributed clustering?

There are many scenarios where distributed clustering algorithms are required. Here are a few examples: 
\begin{itemize}
\item {\em Structural Clustering of web pages from a site}:  Many information extraction tools like wrappers \cite{arasu03extracting, crescenzi01roadrunner} requires as input a set of pages that are created by the same {\em script}. Hence, usually information extraction using wrappers is preceded by a step of {\em site clustering} that clusters the pages in a website into groups of structurally similar pages \cite{crescenzi05clustering, crescenzi02wrapping, charu07xproj}. There algorithms cluster pages based on a number of features drawn from the pages which include HTML dom structure, static text appearing on the page and tokens contained in the urls. Typically one might require hundreds of KB to store all the features of a webpage. Hence, one would require 100 GB - 1 TB of storage to even cluster a site with a million web pages. Clearly in-memory implementations would run out of memory.
    
    Moreover, the number of operations required to cluster a site of 1 M urls could take upto 200 days on a single machine, if the state of the art structural clustering algorithm using single linkage was used \cite{mdlclustering}. We show that, by distributing this load, {\em we can reduce the time taken almost linearly in the number of machines (or some claim like that ...)}
\item {\em Topic Clustering of Pages}: Same as above. The number of documents one might want to cluster now is even larger -- tens of billions of pages at a time. And typical topic clustering algorithms maintain a significant amount of local state (a multinomial vector of counts, one per every word in the vocabulary) which could run into 100s of KB. Hence, both in-memory and disk-based algorithms would fail on off the shelf computers.
    
    Moreover, the number of operations is quite large too. In a typical gibbs sampling or collapsed-gibbs sampling algorithm for a typical topic clustering algortihm like LDAs, each sampling step assigns a topic to each word in each document. An algorithm that runs for $t$ iterations would take a total of $t \cdot |D| \cdot |W| \cdot m$ samples if $|D|$  is the number of documents, $|W|$ is the average number of words per document, and $m$ is the number of instructions per sampling step. For $t = 100$, $|D| = 10^10$, $|W| = 1000$ and $m = 10$, we get $10^16$ instructions; a total of 115 days on a 1 GHz machine.
\item {\em Entity Deduplication}: {\em fill in something here ....}
\item {\em Clustering users in a social network}:  While the interaction graph of users can be fit into memory on a single machine, we might want algorithms for distributed clustering in real scenarios because (a) the data is inherently distributed geographically using a system like PNUTS \cite{pnuts}, (b) and if one wants to use other features about users (like profiles, user activity, etc.) for clustering, then one would not want to migrate the least amount of data across data centers (also for "privacy" concerns). 
\end{itemize}



==> clustering/related.tex <==
\subsection{Related Work}
\label{sec:relatedwork}

\begin{table*}[t]
\hspace{-0.2in}
\setlength{\tabcolsep}{2pt}
{\footnotesize
%\begin{tabular}{ |p{1.95cm}|p{1.1cm}|p{1.8cm}|p{1.1cm}|p{1.8cm}|p{1.1cm}|p{1.8cm}|p{0.6cm}|p{1.8cm}|p{1.1cm}|p{1.8cm}| }
\begin{tabular}{ |c|c|c|c|c|c|c|c|c|c|c|  }
  \hline
Name & \multicolumn{2}{|c|}{Transitive Closure} & \multicolumn{4}{|c|}{Agglomerative Clustering}  &\multicolumn{2}{|c|}{Correlation Clustering} &  \multicolumn{2}{|c|}{Inference}
\\ \cline{2-11}
&&&\multicolumn{2}{|c|}{Single-linkage}&\multicolumn{2}{|c|}{Other-linkage}&&&&
\\  \cline{4-7}
& \# of steps & Communication &\# of steps & Communication & \# of steps & Communication & \# of steps & Communication & \# of steps & Communication
%& \# of Steps & Communication & Iter. & Comm. & Iter. & Comm. &  Iter. & Comm. & Iter. & Comm.
\\ \hline
    Pegasus~\cite{pegasus} & $O(d)$  &  $\mathbf{O(N+M)}$ & $O(n)$ & $\mathbf{O(N+M)}$ & -- & --  & -- & -- & O(d) &  $\mathbf{O(N+M)}$  \\ \hline
  Zones~\cite{twiddle} & $O(d)$ & $\mathbf{O(N+M)}$ & $O(n)$ & $\mathbf{O(N+M)}$ & -- & -- & --  & -- & -- & --\\ \hline
  L Datalog~\cite{foto11:recursive} & $O(d)$ & $ O(nN+M)$  & -- & -- & -- & -- &  -- & -- & -- & --\\ \hline
  NL Datalog~\cite{foto11:recursive} & $\mathbf{O(\boldsymbol\log{d})}$ & $ O(nN+M)$  & -- & -- & -- & -- & -- & -- & -- & --\\ \hline
   $\ha$& $\mathbf{O(\boldsymbol\log{d})}$ & $O(n^2N +M)$ & $\mathbf{O(\boldsymbol\log{n})}$ &  $O(n^2N+M)$ & $\mathbf{O(\boldsymbol\log{n})}$ &  $\mathbf{O(n^2N +M)}$ & $\mathbf{O(n)}$ &  $O(n^2N+M)$ & $\mathbf{O(\boldsymbol\log{d})}$ &   $O(n^2N +M)$\\ \hline
  $\hm$ & $\mathbf{O(\boldsymbol\log{d})}$ & $\mathbf{O(N+M)}$ & $\mathbf{O(\boldsymbol\log{n})}$ &  $\mathbf{O(N+M)}$ & -- & -- & $\mathbf{O(n)}$ & $\mathbf{O(N+M)}$ & -- &  --\\
  \hline
\end{tabular}
}
\caption{Complexity comparison of our results with related work. Best bounds in each column are shown in bold. -- appears whenever a technique is not applicable for a problem. $\hm$ has the best bounds among all techniques, except for other-linkage agglomerative and inference problems, where it is not applicable. For those two problems, $\ha$ gives best bounds. }
\end{table*}


\eat{
\begin{table*}[t]
\hspace{-0.35in}
\begin{tabular}{ |p{2.2cm}|p{1.2cm}|p{2.25cm}|p{1.2cm}|p{2.25cm}|p{1.2cm}|p{2.25cm}|p{1.2cm}|p{2.25cm}|p{1.2cm}|p{2.25cm}|  }
  \hline
 \multirow{2}{*}{Name} & \multicolumn{2}{|c|}{Transitive Closure} & \multicolumn{2}{|c|}{Single-linkage} & \multicolumn{2}{|c|}{General-linkage}  &\multicolumn{2}{|c|}{Correlation Clustering} &  \multicolumn{2}{|c|}{Inference} \\ \cline{2-11}
   & Iterations & Comm. & Iterations & Comm. &  Iter. & Comm. & Iterations & Comm.\\
   \hline
  Pegasus~\cite{pegasus} & $O(d)$  &  $\mathbf{O(N+M)}$ & $O(n)$ & $\mathbf{O(N+M)}$ & -- & -- & -- & -- & O(d) &  $\mathbf{O(N+M)}$  \\ \hline
  Zones~\cite{twiddle} & $O(d)$ & $\mathbf{O(N+M)}$ & $O(n)$ & $\mathbf{O(N+M)}$ &  -- & -- & -- & -- & -- & --\\ \hline
  L Datalog~\cite{foto11:recursive} & $O(d)$ & $ O(\sum_i N_i^2+M)$ & -- & -- & -- & -- &  -- & -- & -- & --\\ \hline
  NL Datalog~\cite{foto11:recursive} & $\mathbf{O(\boldsymbol\log{d})}$ & $ O(\sum_i N_i^2+M)$ & -- & -- & -- & -- -- & -- & -- & --\\ \hline
    $\ha$~(Sec.~\ref{hashing}) & $\mathbf{O(\boldsymbol\log{d})}$ & $O(\sum_i N_i^3 +M)$ & $\mathbf{O(\boldsymbol\log{n})}$ &  $O(\sum_i N_i^3 +M)$ & $\mathbf{O(\boldsymbol\log{n})}$ &  $\mathbf{O(\sum_i N_i^3 +M)}$ & $\mathbf{O(n)}$ &  $O(\sum_i N_i^3 +M)$ & $\mathbf{O(\boldsymbol\log{d})}$ &   $O(\sum_i N_i^3 +M)$\\ \hline
  $\hm$~(Sec.~\ref{hashing}) & $\mathbf{O(\boldsymbol\log{d})}$ & $\mathbf{O(N+M)}$ & $\mathbf{O(\boldsymbol\log{n})}$ &  $\mathbf{O(N+M)}$ & -- & -- & $\mathbf{O(n)}$ & $\mathbf{O(N+M)}$ & $\mathbf{O(\boldsymbol\log{d})}$ &  $\mathbf{O(N+M)}$\\

  \hline
\end{tabular}
\caption{Complexity comparison of our results with related work. Best bounds in each column are shown in bold.}
\end{table*}
}

%\subsection{Centralized Algorithms}

%\subsection{Distributed Transitive Closure and Connected Components}

Finding connected components in a distributed setting is well studied problem. In 1976, Hirschberg~\cite{hirschberg76:tc} proposed a parallel approach based on the simple idea that given a graph represented by its adjacency matrix $M$, its transitive closure is the graph corresponding to the matrix $M^{d}$, where $d$ is the longest diameter of any connected component. The method computed $M^{d}$ iteratively by repeated squaring and thus finished in $O(\log{d})$ iterations. However, it predated Map-Reduce and assumed a shared memory for storing the matrix that was accessible by all processors; there is no direct way to extend their algorithm for non-shared memory. Furthermore since the graph was represented as a matrix, the communication complexity was $O(\nnodes^2)$, quite reasonable at that time, but certainly intolerable for modern-day large graphs.

Google's MapReduce lecture series describes an iterative approach for computing connected components. In each iteration a series of map-reduce steps are used to find and include all nodes adjacent to current connected components. The number of iterations required for this method is thus $O(d)$ where $d$ is the diameter of the largest connected-component. Various methods~\cite{pegasus,twiddle,mpi} have subsequently been proposed that reduce the work done per iteration bringing down communication per iteration from Hirschberg's $O(\nnodes^2)$ to $O(\nnodes+\nedges)$~(a big saving for sparse graphs where $\nedges << \nnodes^2$). However, all these methods expand the connected components one layer of adjacent nodes at a time, and can be though of as computing $M^{d}$ through repeated multiplication by $M$, and thus require $O(d)$ iterations. Since the diameter of most graphs in practice is small ($\leq 20$), the methods are considered quite practical. For large diameter graphs (such as graphical models where edges represent correlations between variables), or for more general forms of clustering (where fixed point occurs at higher powers of $M$ rather than $M^{d}$), such methods of iterative matrix multiplication are not feasible.

Our connected components algorithm follows Hirschberg's approach of repeated squaring (rather than repeated multiplication) and thus finishes in $O(\log{d})$ iterations. However, as we keep on squaring, the matrices become less and less sparse, which will increase the communication complexity. In a central setting, this can be handled by observing that even though the matrix is less sparse, a connected component of size $n$ can be stored as a single cluster of size $n$, rather than $n^2$ 1's in the adjacency matrix. Matrix squaring can then be thought of as merging overlapping clusters. However, in a distributed setting, a naive approach for merging overlapping clusters, might require the clusters to be replicated and moved around. This is where our efficient hashing and merging logic comes in and keeps the communication complexity to $O(\nnodes+\nedges)$.

\eat{
Copied from \cite{twiddling}: ''GoogleÕs MapReduce lecture series describes a simple MapReduce approach to component finding.2 This method does the obvious: it starts from a specified seed vertex s, uses a MapReduce job to find those vertices adjacent to s, compiles the updated vertex information in another MapReduce job, then repeats the process, each time using two MapReduce jobs to advance the frontier another hop. If the graph consists of a single component, this approach will take $2\epsilon(s)$ MapReduce jobs, where $\epsilon(v)$ is the eccentricity of $v$. (The eccentricity of a vertex is the maximum distance from that vertex to another vertex in the graph.)"

Zone-based approach of \cite{twiddling,mpi}: ''The algorithm begins (before the iteration loop) by assigning each vertex to its own component or Òzone,Ó  Each iteration grows the zones, one layer of neighbors at a time. As zones collide due to shared edges, a winner is chosen (the smaller zone ID), and vertices in the losing zone are reassigned to the winning zone. When the iterations complete, each zone has become a fully connected component. The algorithm thus finds all connected components in the graph simultaneously. The number of iterations is linear in the largest diameter of any component in the graph."

Pegasus approach \cite{pegasus}: ''The main idea is as follows. For every node $v_i$ in the graph, we maintain a component id $c^h_i$ which is the minimum node id within $h$ hops from $v_i$. Initially, $c^h_i$ of $v_i$ is set to its own node id: that is, $c^0_i$ = $i$. For each iteration, each node sends its current $c^h$ to its neighbors. Then $c^{h+1}$, component id of $v_i$ at the next step, is set to the minimum value among its current component id and the received component ids of its neighbors. Again the number of iterations is linear in the largest diameter of any component in the graph. communication complexity per iteration is O(E)"




\subsection{Distributed Clustering}



\subsection{Other Distributed Algorithms}

Papers about mapreduce for coclustering and k-means clustering. But they are quite trivial and different. They are:
\begin{itemize}

\item1. DisCo: Distributed Co-clustering with Map-Reduce

\item 2. MapReduce for Sparse Graph Algorithms

\item http://alex.smola.org/papers/2010/SmoNar10.pdf

\end{itemize}
}

==> clustering/results.tex <==
\subsection{Results}

Let $\machine{e}$ denote the machine corresponding to entity $e$.

\begin{theorem}[Transitive Closure] The number of map-reduce iterations required for $\DC(\ha)$ to compute transitive closure is at most $\log{d}$, where $d$ is the diameter of the largest connected component in the transitively closed graph.
\end{theorem}
\begin{proof} We prove the result using induction. Let $T(e) \in F_e$ be the current tree containing entity $e$ in the machine $\machine{e}$.  Also denote $\Delta(e,x)$ the shortest path length from $e$ to $x$ in the original graph $G$, The inductive hypothesis is as follows:

$$IH(k)= \forall e,x: \Delta(e,x) \leq 2^k \Rightarrow x \in T(e)$$

$IH(0)$ is trivially true since $\DC$ sends $F_e$ containing each neighbor of $e$ to $\machine{e}$.

Assume $IH(k)$ is true. To prove $IH(k+1)$, take any node $y$ such that $\Delta(e,y) \leq 2^{k+1}$. Let $x$ denote the midpoint of a shortest path between $e$ and $y$. Then $\Delta(e,x) \leq 2^{k}$ and $\Delta(e,y) \leq 2^{k}$. By $IH(k)$, $e,y \in T(x)$. In step k+1, \Ha will send $T(x)$ to node $e$ and therefore $e,y$ will be in $T(e)$ at the end of this step. This proves $IH(k+1)$.

\end{proof}


\eat{
\begin{theorem}[Transitive Closure] The number of map-reduce iterations required for $\D_{TC}(\hm)$ is at most $2\log{d}$, respectively, where $d$ is the diameter of the largest connected component in the original graph.
\end{theorem}
\begin{proof}

We show that each step of $\DC$ with \Ha is simulated by two steps of \Hm. Let a new cluster $C$ be formed in a step of \Ha by combining clusters $C_1, C_2, \ldots$ from the previous step. Therefore we need that there is at least one node $x\in \bigcap_i C_i$. Suppose $C_1, C_2, \ldots$ are {\em computed} by \Hm in Step-0:  A cluster $C_i$ is said to be computed in \Hm if denoting $m_i = min(C_i)$, $C_i$ occurs in the machine $\machine{m_i}$ and $m_i$ occurs in all nodes in $C_i \cup \n(C_i)$.

Then two steps of \Hm have the following effect:

\begin{enumerate}
\item {\bf Move Min:} In the first step the minimum node $m* = \min_i m_i$ is computed on $\machine{x}$. Then, $m*$ is sent to every $\machine{m(i)}$. Note that $\machine{m(i)}$ knows the entire cluster $C_i$.
\item {\bf Move All:} In the second step, each $C_i$ is moved from $\machine{m(i)}$ to $\machine{m*}$ and $m*$ is sent to each $\machine{x}$ for each $x\in \bigcup_i C_i$. Therefore $C=\bigcup_i C_i$ is computed (locally at $\machine{m*}$).
\end{enumerate}
\end{proof}


\begin{theorem} For any agglomerative clustering algorithm $\cal AC$ and stopping predicate $\Stop$, the number of map-reduce iterations required for $\DC_{\cal AC}(\hm,\Stop)$ is at most $2$ times the number of iterations for $\DC_{\cal AC,\Stop}(\ha)$.
\end{theorem}
\begin{proof}

We show that each step of $\DC$ with \Ha is simulated by two steps of \Hm. Let a new cluster $C$ be formed in a step of \Ha by combining clusters $C_1, C_2, \ldots$ from the previous step. Therefore we need that there is at least one node $x \in \bigcap_i C_i \cup \n(C_i)$. Suppose $C_1, C_2, \ldots$ are {\em computed} by \Hm in Step-0. A cluster $C_i$ is said to be computed in \Hm if denoting $m_i = min(C_i)$, $C_i$ occurs in the machine $\machine{m_i}$ and $m_i$ occurs in all nodes
The \Hm algorithm performs two steps:

\begin{enumerate}
\item {\bf Move Min:} In the second step the minimum node $m* = \min_i m(i)$ is computed on $\machine{x}$. Then, $m*$ is sent to every $\machine{m(i)}$. Note that $\machine{m(i)}$ knows the entire cluster $C_i$.
\item {\bf Move All:} In the final step, each $C_i$ is moved from $\machine{m(i)}$ to $\machine{m*}$ and $m*$ is sent to each $\machine{x}$ for each $x\in \bigcup_i C_i$. Therefore $C=\bigcup_i C_i$ is computed (locally at $\machine{m*}$).
\end{enumerate}
\end{proof}
}

\eat{
Next we prove the result for \Hm.  Let $m$ be the minimum element in the connected component of diameter $n$. We need to prove that it will be computed in $3\log{n}$ steps. The inductive hypothesis ($IH(k)$) that we uses states that any connected component that contains $m$ and has diameter $2^k$ is computed in at most  $k$.  By computing, we mean that the connected component appears as a node in the forest of the machine $m$ and each machine corresponding to the entity $e$ in the forest contains the minimum element $m$.  $IH(1)$ is trivially true since \Hm\  will send to machine $m$, each pair of nearest neighbors of $m$, and also send $m$ to each of the machines corresponding the nearest neighbors of $m$.  Hence $2^{1}$ diameter connected components containing $m$ are computed in iteration $1$.

Assume $IH(k)$ is true. Hence at time $k$ we have all connected components of diameter $2^k$ containing $m$ computed. To prove $IH(k+1)$, take any connected component $cc$ containing $m$ of diameter $2^{k+1}$. Then $cc$ can be thought of as the union of two connected components $cc_1$ and $cc_2$ of diameters $2^{k}$ each (simply split $cc$ in the middle of its longest path).  We also  know that at least one of those components contains $m$. W.L.O.G, assume that $cc_1$ contains $m$. Also denote $m_2 = min(\nn{\nodes{F_2}}{\D})$. We know by $IH(k)$ that $cc_1$ and $cc_2$ are computed in some machines at time $3k$.

 Let $(e_1,e_2)$ be the edge that  connects $cc_1$ and $cc_2$, respectively, to form $cc$. In iteration $3k+1$, \Hm\ will hash $m$ to $e_2$, since $e_1$ contains $m$ and \Hm\ sends the min element  to nearest neighbors of $e_1$.  In iteration $3k+2$, \Hm\ will hash $m$ to machine $m_2$, since $e_2$ contains forest having both $m$ and $m_2$, and thus the  minimum element $m$ will be sent to all nearest neighbors including $m_2$. In iteration $3k + 3$, the forest at $m_2$ will be sent to $m$, where it will be merged with the forest of $m$ and thus $cc$ will appear as a node in the forest of $m$ Also $m$ will be sent to each element in the forest of $m_2$. STUCK HERE SINCE ITERATION $3k+3$ ASSUMES THAT THE FOREST OF $m_2$ REMAINS AT MACHINE $m_2$. ACTUALLY IT MIGHT HAVE MOVED TO SOME OTHER MACHINE WITH A LOWER ID. ONE SIMPLE SOLUTION IS TO MODIFY THE ALGORITHM SO THAT FORESTS ARE MOVED EVERY THIRD STEPS ONLY


\begin{proposition}[Single-linkage Spanning Tree] \label{prop:spanning} Any run of a single-linkage algorithm corresponds to a spanning tree over the graph with nodes in entities $E$  and edges in nearest neighbor edges between $E$. The spanning tree has the property that any edge $(e_1,e_2)$ in the tree has distance less than any edge incident on $e_1$ or $e_2$ that does not lie in the tree
\end{proposition}
}

\begin{theorem}[Single-linkage Runtime] \label{thm:single:linkage} Given set of entities $E$, centralized algorithm ${\cal A}({\cal D},{\cal P}, \Stop)$  creating $\C$, consider the hash-to-all distributed algorithm $\DC(\ha,\M_\A,\Stop)$ corresponding to $\A$. That algorithm terminates in $\lfloor \log{n} \rfloor$ map-reduce steps if $\Stop$ is local and monotonic. Also $\DC(\hm,$ $\M_{\A},$ $\Stop)$ terminates in $3 \lfloor \log{n} \rfloor$ steps.
\end{theorem}

\begin{proof} To prove Theorem~\ref{thm:single:linkage}, we first define the notion of golden clustering.
\end{proof}

\begin{definition}[Golden Clustering]
Consider a set $E$ of entities, and a centralized algorithm ${\cal A}({\cal D},{\cal P}, \Stop)$ (as defined previously) that creates a clustering ${\cal C}$. We say that a clustering ${\cal C}_g$ (not necessarily disjoint) of $E$ is a {\em golden clustering} of $E$ w.r.t. ${\cal A}$ iff
$$\forall C_g \in {\cal C}_g, \exists C \in {\cal C} \mbox{ s.t. } C_{g} \subseteq C$$
%$\forall C_g \in {\cal C}_g, \forall C_{core} \in MCD(C_g), \exists C \in {\cal C} \mbox{ s.t. } C_{core} \subseteq C$.
\end{definition}

\begin{lemma}[Nearest neighbor to a Golden Cluster] \label{lemma:nngc}
Given set of entities $E$, centralized algorithm ${\cal A}$ creating ${\cal C}$, let  ${\cal C}_g$ be a golden clustering of $E$ w.r.t ${\cal A}$.  Then for every $C_{g} \in {\cal C}_g$, denoting $C\in \C$ the cluster in $\C$ that is the superset of $C_g$, there exists $C_n \in NN(C_g)$ such that $C_n \subseteq C$.  (Define $NN$ to take a cluster and return all nearest-neighbor clusters and $Nn$ to return the unique nearest-neighbor element.)
\end{lemma}
\begin{proof}   We will first show that $Nn(C_g) \in C$. Assume the contrary: $Nn(C_g) = d \notin C$. Therefore, there exists $b \in C_g$ such that $\D(b,d)$ be the nearest-neighbor edge between $C_g$ and $E$. In other words, $\D(b,d) < \min_{a \in C_g, x \in C \setminus C_g} D(a,x)$. Now consider the iteration of the centralized algorithm when it merged a subset of $C_g$ containing $b$ to form a superset of $C_g$. Let the nearest-neighbor edge for that iteration be $(p,q)$, therefore $p \in C_g$ and $q \in C \setminus C_g$. Then $D(p,q) < D(b,d)$ which contradicts the above inequality. This shows $Nn(C_g) \in C$.

To prove the above lemma, note that since $\C_g$ is a clustering, there exists a cluster $C_n \in \C_g$ that contains $Nn(C_g)$. Since $C_n \cap C$ contains $Nn(C_g)$, $C_n$ overlaps with $C$, and hence $C_n \subseteq C$. This proves the lemma.
\end{proof}

\begin{lemma}[Existence of Golden Clustering]
Given a set of entities $E$, centralized algorithm ${\cal A}$ creating ${\cal C}$, consider the Hash-to-All distributed clustering algorithm $\DC(\ha,$ $\M_{\A},$ $\Stop)$ corresponding to $\A$, let the cluster on machine $v \in V$ in iteration $k$ of $\DC$ be $C_v(k)$. Then there exists a subset of machines $V_g(k) \subseteq V$  for each $k$ such that (i) if we define ${\cal C}_g(k) = \cup_{v \in V_g(k)} MCD(C_v(k))$, then ${\cal C}_g(k)$ is a golden clustering of $E$ w.r.t ${\cal A}$, and (ii) $|V_g(k+1)| \leq |V_g(k)|/2$.
\end{lemma}
\begin{proof}
We prove the lemma by induction on $k$.

\begin{itemize}
\item {\bf $k=1$:} We have ${\cal C}_k  = \{ \{e\} | e\in E\}$. Therefore, ${\cal C}_g(1)={\cal C}_k$ is a golden clustering w.r.t $\C$.

\item {\bf $k\rightarrow (k+1)$:} Suppose we have a golden clustering ${\cal C}_g(k)$ in iteration $k$. % as cores in the set $V_g(k)$ of machines after $k$ steps.
Denote $critical(C_v) \in MCD(C_v)$ the core that is closest to its nearest neighbor, i.e  equals $$argmin_{C_{core} \in MCD(C_v)} Dist(C_{core},NN(C_{core}))$$
Denote $NN(v) = min_{e} \{ e : \exists e'  \in Nn(critical(C_v))\}$.  Thus $NN$ forms a directed graph on node set as $V_g(k)$ and nearest neighbor as directed edges. Each node $v$ has exactly one outgoing edge $NN(v)$. Each connected component in the graph has exactly one 2-cycle~(i.e. nodes $v,v'$ such that $NN(v_2) = v_1$ and $NN(v_1)=v_2)$. For all other nodes $v$, there exists a unique path of outgoing edges using at most one edge of the 2-cycle to both $v_1$ and $v_2$. Let $V_1$~($V_2$) be the set of nodes $v$ that are closer to $v_1$~($v_2$) than $v_2$~($v_1$). Define for each node $v$ in $V_1$~($V_2$), $level(v)$ as the path length of $v$ from $v_1$~($v_2$). Thus $v_1$ and $v_2$ have level $0$ and all other nodes have level $\geq 1$. Denote $even(V_1)$~($even(V_2)$) the set of nodes with level as an even number in $V_1$~($V_2$). Similarly define $odd(V_1)$~($odd(V_2)$). Then we define $V_g(k+1)$ as the smaller of the two sets: $odd(V_1) \cup even(V_2)$ or $odd(V_1) \cup even(V_2)$.


It is easy to see that from its construction, $|V_g(k+1)| \leq |V_g(k)|/2$. All that remains to be proven is that   ${\cal C}_g(k+1) = \cup_{v \in V_g(k+1)} MCD(C_v(k+1))$ is a golden clustering. First we claim that for each $v \in V_g(k)$, either $v$ or $NN(v)$ exists in  $V_g(k+1)$. This is true simply because of and $level(NN(v)) = level(v) + 1$ and hence have different odd/even parities. Moreover, \Ha will send for each $v \in V_g(k)$ the cluster $C_v(k)$ to both machines $v$ and $NN(v)$ in the $(k+1)^{th}$ iteration. Hence $V_g(k+1)$ will always have the cluster $C_v(k)$ on some machine, either alone or along with other clusters. Thus $\C_g(k+1)$ is a clustering. To show that is golden, assume that the merge step on any machine, we merge two or more overlapping clusters to get a cluster $C_v(k+1)$. According to the stopping lemma (ADD LEMMA), we know for all $C_{core} \in MCD(C_v(k+1))$, $\Stop(C_{core})=0$. In other words, each $C_{core}$ in the set $\cup_{v \in V_g(k+1)} MCD(C_v(k+1))$ is a valid core. Hence ${\cal C}_g(k+1) = \cup_{v \in V_g(k+1)} MCD(C_v(k+1))$ is a golden clustering.

\end{itemize}
\end{proof}




%\begin{proof}


\eat{
[[Need to change the proof]]
Let $C$ be the largest cluster. The proof is by induction on the size of $n$. Let $T$ be the spanning tree on $C$.  Let $(e_1,e_2)$ correspond to the largest distance edge in $S$. Then removing the edge breaks the tree in two trees $T_1$ and $T_2$. Let $C_1$ and $C_2$ be the clusters corresponding to the trees $T_1$ and $T_2$, respectively. W.L.O.G, there are two possible cases:
\begin{enumerate}
\item $|C_1| = |C_2| = n/2$: Then by IH, both  $C_1$ and $C_2$ are computed in $\lfloor \log{n} \rfloor -1$ steps. Furthermore since $(e_1,e_2)$ is an edge in the spanning tree $T$, by Proposition~\ref{prop:spanning}, it is the nearest neighbor edge that lies outside the clusters $C_1$ and $C_2$. Hence \Ha will map $C_1$ and $C_2$ to the same machine in the next iteration that will yield $C = C_1 \cup C_2$ in $\lfloor \log{n} \rfloor$ iterations.

\item $|C_1| > n/2$: Then by IH, $C_2$ is computed in $\lfloor \log{n} \rfloor -1$ steps.  Furthermore since $(e_1,e_2)$ is an edge in the spanning tree $T$, by Proposition~\ref{prop:spanning}, it is the nearest neighbor edge that lies outside the cluster $C_2$. Hence \Ha will map  $C_2$ to machine $e_1$ in the next iteration. Similarly, $C_1$ will be computed on $e_1$ in time $\lfloor \log{n} \rfloor$ by IH. (NOT TRUE, IH DOESN"T QUITE WORK)
\end{enumerate}
 }

%\end{proof}

Theorem 2 (Anish):  Matching lower bound? Can we prove this for hash-to-min?

Theorem 3 (?): Any agglomerative algorithm is O(n) for some stopping criterion.

Theorem 4 (hope to prove): something about O(log n) and single-linkage. 

==> proofs/tree_proofs.tex <==
Let $T$ be a tree on nodes $V$. Given a subset of nodes $S \subseteq V$, the subtree $T_s$ induced by $T$ on $S$ has nodes equal to $S$ and edges between any pair of nodes in $S$, that occurs in $T$ if $T_s$ is a connected graph. We denote $root(T_s)$ as the root of $T_s$ corresponding to the node in $S$ which occurs highest in $T$.

\begin{definition}[Local Minima]
A node $v$ is local minimum if all its neighbors have id larger than $v$'s id.
\end{definition}


\begin{definition}[Strictly Increasing] 
A tree is {\em strictly increasing} if for any nodes $a,b$ such that $a$ is ancestor of $b$, $a < b$.
\end{definition}

\begin{proposition} A tree is strictly increasing if and only if it has exactly one local minima at the root.
\end{proposition}
\begin{proof}  To show the if part, assume that $T$ has its only local minima at the root node. To show $T$ is monotone, assume the contrary:  therefore, there exist nodes $a,b$ such that $a$ is $b$'s ancestor and $a > b$.  Now consider the path between $a$ to $b$. Since $a > b$, there exists nodes $c,d$ such that $c$ is the parent of $d$, and $c > d$. Hence the tree is not
\end{proof}


\begin{definition}[Monotone]
A tree is {\em monotone} if only the root nodes and leaf nodes are local minima. That is, the nodes  on every root to leaf path $\ell_0, \ell_1, ..., \ell_k$ are such that one of the following holds:
\begin{itemize}
\item $\ell_0 < \ell_1 < \ldots < \ell_{k-1}$ and $\ell_k < \ell_{k-1}$
\item $\ell_k < \ell_{k-1} < \ldots < \ell_1$ and $\ell_0 < \ell_1$
\end{itemize}
\end{definition}

\begin{lemma}\label{lemma:monotone:tree:size}
Let $T$ be a tree with $n$ nodes each with a randomly chosen id. With probability greater than $1/n^2$ every subtree of $T$ that is monotone has depth less than $4\log{n}$.
\end{lemma}
\begin{proof}
Consider any subtree $T_r$ of $T$ rooted at $r$. There are at most $n$ paths from $r$. In each path, the probability that we have a monotonic sequence of length greater than $4\log{n}$ is at most $2^{-4\log{n}} = 1/n^{4}$. By a union bound, the probability that any path has a monotonic sequence of length greater than $4\log{n}$ is $n \times 1/n^4 = 1/n^3$. Finally, any node $v$ has a monotone subtree rooted at $v$ with depth $> 4\log{d}$ is at most $n \times 1/n^3 = 1/n^2$. Hence proved.
\end{proof}


\eat{Denote $min_k(u)$ the minimum node after $k$ iterations that $u$ knows that also knows $u$. Also denote $\Delta(u,v)$ the distance between node $u$ and $v$.
}



\eat{Thus from above proposition we see that every monotone subtree of $T$ has a root $r$ which is a local minimum in $T$ and vice versa. For a tree graph, we define the notion of levels below.}

\begin{definition}[Level i nodes] Given a tree, level $0$ consists of all nodes in the tree. Level $i$ is then defined recursively as nodes that are local minimum nodes in the subtree of $T$ induced by level $i-1$ nodes. Denote the set of nodes at level $i$ as $level(i)$.
\end{definition}

\begin{definition}[Short-cut and Level i trees] Given a tree $T$, and set of nodes $S$, the short-cut tree $T(S)$ has nodes in $S$ and an edge from a node $v_1$ to $v_2$ if according to $T$, $v_1$ is the closest ancestor to $v_2$ that is present in $S$. A level $i$ tree is a short-cut tree of on nodes $S=level(i)$.
\end{definition}

\begin{proposition} \label{prop:levels} Let $T$ be  a tree of depth $d$. Then for all $i$, the level $i$ tree of $T$ has  $depth \leq d/2^i$.
\end{proposition}
\begin{proof} The proof follows from the fact that for each level $i$, no consecutive nodes can be local minimum. Hence if $P$ is any root to leaf path in $T$, then $|P \cap level(i)| \leq |P \cap level(i-1)|/2)$.  Thus $|P \cap level(i)| \leq length(P)/2^i$. Also the length of path $P'$ in the level i tree corresponding to path $P$ in $T$ is exactly $P \cap level(i)|$.  Hence the depth of level $i$ tree is $\leq d/2^i$, which implies our claim.
\end{proof}


\begin{theorem} \Hm finishes on a tree of depth $d$ in time $2\log{d}\log{\log{n}}$ iterations with probability greater than $1-1/n$. This probability is over the random choices of the algorithm for deciding the node orderings.
\end{theorem}
\begin{proof}  From lemma~\ref{lemma:monotone:tree:size}, the probability that $T$ has a monotone subtree of depth greater than $4 \log{n}$ is at most $1/n^2$. We also know that \Hm finishes in at most $d \leq n$ iterations. Let $T_i$ be the shortcut tree induced by set of minimum nodes (considering min at every cluster) after iteration $i$. By a union bound, the probability that every $T(i)$ has a monotone subtree of depth greater than $4\log{n}$ is at most $d/n^{2} \leq  n/n^2 \leq 1/n$. Hence with probability greater than $1 - 1/n$, we can assume that all trees T(i) have all monotone subtrees of depth less than $4\log{n}$.

By Lemma~\ref{lemma:tree:levels} we know that after $k = \log{4\log{n}} = 2 + \log{\log{n}}$ iterations, only level $1$ nodes can be the minimum nodes at any cluster. Thus the tree $T(k)$ is a subtree of the level 1 tree, and hence has depth less than $d/2$. Thus in $k=\log{\log{n}}$ iterations, the depth $d$ of tree $T=T(0)$ reduces to $d/2$ of tree $T(k)$. Thus the total number of iterations is bounded by $2\log{d}\log{\log{n}}$.  Hence proved.
\end{proof}


\begin{lemma} \label{lemma:tree:levels}  If $d_0$ is the depth of  monotone subtree of $T$ with largest depth, then in $\log{d_0}$ iterations of \Hm the minimum at every node is a level 1 node.
\end{lemma}
\begin{proof}
\red{to do: if helpful see the lemma below}
\end{proof}


\begin{lemma}\label{lemma:tree}
Consider a monotone tree T with root $m$. Then after $k$ iterations of the Hash-to-min algorithm,
\begin{itemize}
\item For every node $j$ within a distance of $2^k$ from the minimum node $m$, $m$ knows $j$ and $j$ knows $m$.
\item For every pair of nodes $i, j$ such that $i$ is ancestor of $j$, and are at a distance $2^k$ apart, $i$ knows $j$ and $j$ knows $k$.
\item Node $j$ is not known to and does not know any node $i$ that is at a distance $>2^k$.
\end{itemize}
\end{lemma}
\begin{proof}
The proof is by induction. \\
{\em Base Case:} After 1 iterations, each node knows about its 1-hop and does not know 2-hop neighbors (on either side).  \\
{\em Induction Hypothesis:} Suppose the claim holds after $k-1$ iterations. \\
{\em Induction Step:} \\
In the $k^{th}$ iteration, consider a node $j$ that is at a distance $d$ from the min node $m$, where $2^{k-1} < d \leq  2^k$. From the induction hypothesis, there is some node $i$ that is $2^{k-1}$ away from $j$ that knows $j$. Since, $m$ is known to $i$ (from induction hypothesis), the Hash-to-min algorithm would send $j$ to $m$ and $m$ to $j$ in the current iteration. Therefore, $m$ knows $j$ and $m$ is known to $j$.

Consider a node $j$ that is $>2^k$ distance from the min node. At the end of the previous iteration, $j$ knew (and was known to) $i$, and $i$ knew and was known to $i'$ -- where $i$ and $i'$ are at distance $2^{k-1}$ from $j$ and $i$ respectively. Moreover, $i$ did not know any node $i''$ smaller than $i'$. Therefore, in the current iteration, $i$ sends $i'$ to $j$ and $j$ to $i'$. Therefore, $j$ knows and is known to a node that is $2^k$ distance away.

Finally, we can show that a node does not know (and is not known to) any node that is distance $>2^k$ as follows. Node $j$ can only get a smaller node $i'$ if $i'$ is a minimum at some node $i$. Since in the previous step no one knows a node at distance $>2^{k-1}$, $j$ cannot know a node at distance $>2^k$.
\end{proof}




==> proofs/vibhor_proofs.tex <==

Denote $min_k(u)$ the minimum node after $k$ iterations that $u$ knows that also knows $u$. Also denote $\Delta(u,v)$ the distance between node $u$ and $v$.
\begin{definition}[Local Minima]
A node $v$ is local minimum if all its neighbors have id larger than $v$'s id.
\end{definition}

For a path graph, we define the notion of levels below.

\begin{definition}[Levels] Given a path, level $0$ consists of all nodes in the path. Level $i$ is then defined recursively as nodes that are local minimum nodes among the nodes at level $i-1$, if the level $i-1$ nodes are arranged in the order in which they occur in the path. Denote the set of nodes at level $i$ as $level(i)$.
\end{definition}

\begin{proposition} \label{prop:levels:number} The number of levels having more than $1$ node is at most $\log{n}$.
\end{proposition}
\begin{proof} The proof follows from the fact that for each level $i$, no consecutive nodes can be local minimum. Hence $|level(i)| \leq |level(i-1)/2)$.
\end{proof}

\begin{lemma}\label{lemma:path:levels}
Consider a path $P$ with three segments $P_1, P_2$ and $P_3$, where $P_1$ and $P_3$ are arbitrary, and $P_2$ has $r+1$  level $\ell$ nodes $l_1,l_2,...l_r,m_1$  going from left to right. Assume that labels are such that $l_1 < l_2 < \ldots < l_r$.  For a node $l_i$, denote $\lr(l_i,k,\ell)$ the closest level $\ell$ node $l_j$ from $l_i$ towards the right such that $min_k(l_j) > l_i$. Denote $T(k,\ell)$ and $M(k,\ell)$ as $$T(k,\ell) = min_{P,l_i: \lr(l_i,k,\ell) \neq l_r} \Delta(l_i,\lr(l_i,k,\ell))$$ and $$M(k,\ell) = min_{P: min_k(l_1) > min_{k-1}(m_1)\mbox{ or }min_k(m_1) > min_{k-1}(l_1)} \Delta(l_1,m_1)$$.

Then the following is true:
\begin{enumerate}

\item If $min_{k-1}(l_i) \leq l_1$ then $min_k(l) \leq l$.

\item $T$ satisfies the following recurrence realtion
            \begin{eqnarray*} 
              T(k,\ell) \geq min(T(k-2,\ell) + min(T(k-1,\ell), M(k,\ell)), \\ M(k-1,\ell-1) 
             \end{eqnarray*} 
             
\item $M$ satisfies the following recurrence relation
        \begin{eqnarray*}
           M(k,\ell) \geq  min(T(k-2,\ell),M(k-1,\ell-1))
        \end{eqnarray*}
        
\end{enumerate}

\end{lemma}


\begin{proof}
\eat{
{\em Base Case (k=2):}  We know that after 2 iterations any local minimum node $l_i$ would be the minimum node for $l_j$, if $l_j$ exists (i.e $l_i$ is not $l_r$) and $\Delta(l_i,l_j)$ is 2.  This is because in iteration 1, the node $u$ that is between $l_i$ and $l_j$ gets both nodes. Hence the min at $u$ after $1$ iteration is $l_i$. Thus in iteration 2, $l_i$ will be sent to $l_j$ and $l_j$ to $l_i$. Hence $min_2(l_j) = l_i$. Thus $\lr(l_i,2)$ has to be greater than $2 = 2^{2-1}$.  \\

{\em Induction Hypothesis :}   For all $l_i$, if $\lr(l_i,k-1)$ is not $l_r$, then $\Delta(l_i,\lr(l_i,k)) > 2^{k-2}$. \\

{\em Induction Step:}
}

Denote by $[l_t,l_u]$ the level  $\ell$ nodes between $l_t$ and $l_u$, and $[l_t,l_u)$ those nodes except for $l_u$.

{\bf Proof of claim 1:} TO ADD

{\bf Proof of claim 2:} Let $l_s = \lr(l_i,k-1,\ell)$ and let $l_t$ be the level $\ell$ node just to the left of $l_s$. We know by definition of $l_s=\lr(l_i,k-1,\ell)$ that  $min_{k-1}(l_s) >  l_i$, but for all $l \in [l_i,l_t], min_{k-1}(l) \leq l_i$. Now there are three cases:

\begin{enumerate}
\item $min_{k-1}(l_t) \in P_3$. Then $min_{k-1}(l_t) \leq l_i$~(from above), and any node $l \in [l_t,l_r]$ would have $min_{k-1}(l) \in P_3 \leq min_{k-1}(l_t)$. Hence $\min_{k-1}(l) \leq l_i$ for all $l \in \{l_i,\ldots,l_r\}$. Thus $\lr(l_i,k-1) = l_r$.

\item $min_{k-1}(l_t) \notin P_3$ and $\Delta(l_i,l_t) \geq T(k-1,\ell)$. Denote $l_u =  \lr(l_t,k-1,\ell)$.  Consider any $l \in [l_t,l_u)$. Let $a=min_{k-1}(l)$. Then from the definition of $l_u =  \lr(l_t,k-1)$ and since $l \in [l_t,l_u)$, we know that, $a = min_{k-1}(l) \leq l_t$. Now there are two sub-cases: 

\begin{enumerate} 
\item For all $l \in [l_t,l_u)$, $a = min_{k-1}(l)  \notin P_3 \cup \{m_1\} $. In this case, we show that $\lr(l_i,k,\ell)$ is a level $\ell$ node in $[l_u,l_r]$. For this we will show that for all $l \in [l_t,l_u)$ and $a = min_{k-1}(l)$,  $min_{k-1}(a) \leq l_i$.  If $a \notin P_3 \cup \{m_1\}$, then either (i) $a \in P_1$, in which case  $a \leq l_1$~(otherwise $min_{k-1}(l)$ would be $l_1$ and not $a$), and hence obviously $min_{k-1}(a) \leq l_i$, or (ii) $a in P_2$ but $a \neq m_1$, and then since $a \leq l_t$~(from above), $a \in [l_i,l_t]$. Hence $min_{k-1}(a) \leq l_i$. 

In other words, after $k-1$ iterations, the minimum for any node $l \in [l_t,l_u)$ is $a$, which in turn has a minimum $b \leq l_i$. Thus in one \Hm step, $b$ would become $min_k(l)$. Hence after $k$ iterations and for any local minimum $l$ between $l_i$ and $l_u$, we have $min_k(l) \leq l_i$.  This shows that $\lr(l_i,k,\ell) \in [l_u,l_r]$. Then either $l_u$ is $l_r$ or the following holds.
 
$$ \Delta(l_i,\lr(l_i,k,\ell))  \geq \Delta(l_i,l_t) + \Delta(l_t,l_u) \geq  T(k-2,\ell) + T(k-1,\ell-1)$$

\item  There exists $l \in [l_t,l_u)$, such that $a = min_{k-1}(l)  \in P_3$. Let $l_w = \lr(l_i,k,\ell)$. Then $l_w$ is the first node in $[l_i,l_r]$ for which $min_{k}(l_w) > l_i$. If $\Delta(l_v,l_w) \leq M(k,\ell)$ then by definition after $k$ iterations $min_k(l_w) \leq min_{k-1}(l_t) \leq l_i$. Thus $\Delta(l_w,l_i) \geq M(k,\ell)$. Thus 
$$ \Delta(l_i,\lr(l_i,k,\ell))  \geq \Delta(l_i,l_t) + \Delta(l_t,l_w) \geq  T(k-2,\ell) + M(k,\ell)$$
\end{enumerate}

\item $min_{k-1}(l_t) \in P_1 || P_2$ and $\Delta(l_i,l_t) \leq T(k-2,\ell)$. In this case, we argue that  $\Delta(l_t,l_s) > M(k-1,\ell-1)$. Assume the contrary: $\Delta(l_t,l_s) \leq M(k-2,\ell-1)$. Since, $\Delta(l_i,l_t) \leq T(k-2,\ell)$, we know that $min_{k-2}(l_t) \leq l_i$. Since $l_t$ and $l_s$ are consecutive level $\ell$ nodes, all the level $\ell-1$ nodes between them are ordered.  Hence by definition of $M(k-1,\ell-1)$, and the fact that $\Delta(l_t,l_s) \leq M(k-1,\ell-1)$, $min_{k-1}(l_s) \leq min_{k-2}(l_t) \leq l_i$ . This contradicts the assumption that $l_s = \lr(l_i,k-1,\ell)$. Thus $\Delta(l_t,l_s) > M(k-1,\ell-1)$.
$$ \Delta(l_i,\lr(l_i,k))  \geq \Delta(l_i,l_t) + \Delta(l_t,l_s) \geq M(k-1,\ell-1) $$
\end{enumerate}

Combining the above cases we complete the proof of claim 1.\\

{\bf Proof of claim 3:}  If $\Delta(l_1,l_r) \leq T(k-2,\ell)$, then $min_{k-2}(l_r) \leq l_1$.  Also if $\Delta(l_r,m_1) \leq M(k-1,\ell-1)$, then $min_{k-1}(m_1) \leq min_{k-2}(l_r) \leq l_1$. If both  $\Delta(l1,l_r) \leq T(k-2,\ell)$ and $\Delta(l_r,m_1) \leq M(k-1,\ell-1)$, then $min_{k-1}(m_1) \leq  l_1$. Hence by claim 1, $min_{k}(m) \leq min_{k-1}(l_1)$. This completes the proof.

\end{proof}

\begin{lemma} \label{lemma:path:cost} Let $T(k,\ell)$ be the quantity as defined in Lemma~\ref{lemma:path:levels}. Then $T(k,\ell) \geq 2^{k/2-\ell}$.
\end{lemma}
\begin{proof} We prove the lemma using induction.

{\em Base Cases: (i) $\ell=0$ and $k\geq1$. Then by  Lemma~\ref{thm:path}, $T(k,0) \geq 2^{k} \geq 2^{k/2 - 0}$. (ii) $k=1$ and $\ell \geq 1$}. For any level $\ell \geq 1$, $T(1,\ell) \geq 1 \geq 2^{1/2-\ell}$.

{\em Induction Hypothesis (IH)} For all $k_0 \leq k-1$ and $\ell_0 \leq \ell-1$,  $T(k_0,\ell_0) \geq 2^{k_0/2-\ell_0}$

{\em Induction Step:} By Lemma~\ref{lemma:path:levels}, we know that:
\begin{eqnarray*}
  T(k,\ell) &\geq& min \left(T(k-1,\ell) + T(k-2,\ell), T(k-2,\ell-1)\right) \\
                 &\geq& min \left(2^{(k-1)/2-\ell} + 2^{(k-2)-\ell}, 2^{(k-2)/2-\ell+1}\right)~~~~\mbox{(using IH)}\\
                 &\geq& min \left(2^{k/2-\ell}(1/2 + 1/\sqrt{2}), 2^{k/2-\ell}\right) \geq 2^{k/2-\ell}\\
\end{eqnarray*}

Hence proved.
\end{proof}


\begin{theorem}\label{thm:main:path} For a path graph with $n$ nodes, the \Hm algorithm ends in $4\log(n)$ steps.
\end{theorem}



\eat{


\begin{lemma}\label{lemma:tree:levels}
Consider a tree with $r$ nodes $l_0,l_1,...l_r$ at level $\ell$. Assume that the tree induced by level $\ell$ is monotone.  For a node $l_i$, denote $\lr(l_i,k,\ell)$ the closest level $\ell$ node $l_j$ in the subtree of $l_i$ such that $min_k(l_j) > l_i$. Also denote $T(k,\ell)$ to be  $min_{l_i: \lr(l_i,k,\ell) \neq l_r} \Delta(l_i,\lr(l_i,k,\ell))$. Then $$T(k,\ell) > min (T(k-1,\ell) + T(k-2,\ell), T(k-2,\ell-1)$$
\end{lemma}

\begin{proof}
\eat{{\em Base Case (k=2):}  We know that after 2 iterations any local minimum node $l_i$ would be the minimum node for $l_j$, if $l_j$ exists (i.e $l_i$ is not $l_r$) and $\Delta(l_i,l_j)$ is 2.  This is because in iteration 1, the node $u$ that is between $l_i$ and $l_j$ gets both nodes. Hence the min at $u$ after $1$ iteration is $l_i$. Thus in iteration 2, $l_i$ will be sent to $l_j$ and $l_j$ to $l_i$. Hence $min_2(l_j) = l_i$. Thus $\lr(l_i,2)$ has to be greater than $2 = 2^{2-1}$.  \\

{\em Induction Hypothesis :}   For all $l_i$, if $\lr(l_i,k-1)$ is not $l_r$, then $\Delta(l_i,\lr(l_i,k)) > 2^{k-2}$. \\

{\em Induction Step:}
}
Let $l_s = \lr(l_i,k-1,\ell)$ and let $l_t$ be the level $\ell$ node which is the closest ancestor of $l_s$. We know by definition of $l_s=\lr(l_i,k-1,\ell)$ that  $min_{k-1}(l_s) > l_i$, but $min_{k-1}(l_t) \leq l_i$. Now there are two cases:

\begin{enumerate}
\item $\Delta(l_i,l_t) \geq T(k-2,\ell)$. Denote $l_u =  \lr(l_t,k-1,\ell)$. Then we argue that $\lr(l_i,k,\ell)$ is $l_r$ or a level $\ell$ node in $l_u$' subtree.  Consider any level $\ell$ node, $l$ between $l_t$ and $l_u$. Let $a=min_{k-1}(l)$. Then from the definition of $l_u =  \lr(l_t,k-1)$ and since $l$ is an ancestor of $l_u$, we know that, $min_{k-1}(l) = a \leq l_t$. Moreover $b=min_{k-1}(l_t) \leq l_i$, for the same reason.  In other words, after $k-1$ iterations, the minimum at $l$ is $a$, which in turn has a minimum $b \leq l_i$. Thus in one \Hm step, $b$ would become $min_k(l)$. Hence after $k$ iterations and for any local minimum $l$ between $l_i$ and $l_u$, we have $min_k(l) \leq l_i$.  This shows that $\lr(l_i,k,\ell)$ is $l_u$ or some local minimum to its right. Then either $l_u$ is $l_r$ or the following holds
$$ \Delta(l_i,\lr(l_i,k,\ell))  \geq \Delta(l_i,l_t) + \Delta(l_t,l_u) \geq T(k-2,\ell) + T(k-1,\ell) $$

\item $\Delta(l_i,l_t) \leq T(k-2,\ell)$. In this case, we argue that  $\Delta(l_t,l_s) > T(k-2,\ell-1)$. Assume the contrary: $\Delta(l_t,l_s) \leq T(k-2,\ell-1)$. Since, $\Delta(l_i,l_t) \leq T(k-2,\ell)$, we know that $min_{k-2}(l_t) \leq l_i$. Since $l_t$ and $l_s$ are consecutive level $\ell$ nodes, all the level $\ell-1$ nodes between them are ordered.  Hence by definition of $T(k-2,\ell-1)$, and the fact that $\Delta(l_t,l_s) \leq T(k-2,\ell-1)$, $min_{k-2}(l_s) \leq l_t$ .  Thus in the next iteration, $min_{k-1}(l_s) \leq l_i$ which contradicts the assumption that $l_s = \lr(l_i,k-1,\ell)$. Thus $\Delta(l_t,l_s) > T(k-2,\ell-1)$.
$$ \Delta(l_i,\lr(l_i,k))  \geq \Delta(l_i,l_t) + \Delta(l_t,l_s) \geq T(k-2,\ell-1) $$
\end{enumerate}

Combining the two cases we can write $T(k,\ell) \geq min (T(k-1,\ell) + T(k-2,\ell), T(k-2,\ell-1))$. Hence proved.
\end{proof}

\begin{lemma}\label{lemma:path:cost} Let $T(k,\ell)$ be the quantity as defined in Lemma~\ref{lemma:path:levels}. Then $T(k,\ell) \geq 2^{k/2-\ell}$.
\end{lemma}
\begin{proof} We prove the lemma using induction.

{\em Base Cases: (i) $\ell=0$ and $k\geq1$. Then by  Lemma~\ref{thm:path}, $T(k,0) \geq 2^{k} \geq 2^{k/2 - 0}$. (ii) $k=1$ and $\ell \geq 1$}. For any level $\ell \geq 1$, $T(1,\ell) \geq 1 \geq 2^{1/2-\ell}$.

{\em Induction Hypothesis (IH)} For all $k_0 \leq k-1$ and $\ell_0 \leq \ell-1$,  $T(k_0,\ell_0) \geq 2^{k_0/2-\ell_0}$

{\em Induction Step:} By Lemma~\ref{lemma:path:levels}, we know that:
\begin{eqnarray*}
  T(k,\ell) &\geq& min \left(T(k-1,\ell) + T(k-2,\ell), T(k-2,\ell-1)\right) \\
                 &\geq& min \left(2^{(k-1)/2-\ell} + 2^{(k-2)-\ell}, 2^{(k-2)/2-\ell+1}\right)~~~~\mbox{(using IH)}\\
                 &\geq& min \left(2^{k/2-\ell}(1/2 + 1/\sqrt{2}), 2^{k/2-\ell}\right) \geq 2^{k/2-\ell}\\
\end{eqnarray*}

Hence proved.
\end{proof}


\begin{theorem}\label{thm:main:path} For a path graph with $n$ nodes, the \Hm algorithm ends in $4\log(n)$ steps.
\end{theorem}
}

\subsection{General Graph Theorem}

In this section, we will show how a run of the \Hm algorithm on a general graph $G$ can be reduced to a run on a chain graph $C$.

\begin{theorem} Let $T(m,n)$  be the first iteration when a node $m$ knows $n$ and $n$ knows $m$ when \Hm is run on graph $G$. Denote $C(m,n)$ as the graph constructed as follows:
\begin{enumerate}
\item Since $m$ and $n$ know each other in $T(m,n)$ steps, there exists a node $c$ that knows $m$ and $n$ in iteration $T(m,n)-1$. Thus
\end{enumerate}
\end{theorem}


